Identifying when Precession can be Measured in Gravitational Waveforms

In binary-black-hole systems where the black-hole spins are misaligned with the orbital angular momentum, precession effects leave characteristic modulations in the emitted gravitational waveform. Here, we investigate where in the parameter space we will be able to accurately identify precession, for likely observations over coming LIGO-Virgo-KAGRA observing runs. Despite the large number of parameters that characterise a precessing binary, we perform a large scale systematic study to identify the impact of each source parameter on the measurement of precession. We simulate a fiducial binary at moderate mass-ratio, signal-to-noise ratio (SNR), and spins, such that precession will be clearly identifiable, then successively vary each parameter while holding the remaining parameters fixed. As expected, evidence for precession increases with signal-to noise-ratio (SNR), higher in-plane spins, more unequal component masses, and higher inclination, but our study provides a quantitative illustration of each of these effects, and informs our intuition on parameter dependencies that have not yet been studied in detail, for example, the effect of varying the relative strength of the two polarisations, the total mass, and the aligned-spin components. We also measure the "precession SNR" $\rho_p$, which was introduced in Refs[1,2] to quantify the signal power associated with precession. By comparing $\rho_p$ with both Bayes factors and the recovered posterior distributions, we find it is a reliable metric for measurability that accurately predicts when the detected signal contains evidence for precession.

==> abstract.tex <==
In binary-black-hole systems where the black-hole spins are misaligned with the orbital angular momentum, precession effects
leave characteristic modulations in the emitted 
gravitational waveform.
Here, we investigate where in the parameter space we will be able to accurately identify precession, for likely observations over coming 
LIGO-Virgo-KAGRA observing runs. Despite the large number of parameters that characterise a precessing
binary, we perform a large scale systematic study to identify the impact of each source parameter 
on the measurement of precession. We simulate a fiducial binary at moderate mass-ratio, signal-to-noise ratio (SNR), and spins, such that
precession will be clearly identifiable, then successively vary each parameter while holding the remaining parameters fixed.  
As expected, evidence for precession increases with signal-to noise-ratio (SNR), higher in-plane spins, more unequal component masses, 
and higher inclination, but our study provides a \emph{quantitative} illustration of each of these effects, and informs our intuition on 
parameter dependencies that have not yet been studied in detail, for example, the effect of varying the 
relative strength of the two polarisations, the total mass, and the aligned-spin components. 
We also measure the ``precession SNR'' $\rho_p$, which was introduced in Refs.~\citep{Fairhurst:2019_2harm, Fairhurst:2019srr} to 
quantify the signal power associated with precession.  By comparing $\rho_p$ with both Bayes factors and the recovered posterior distributions, 
we find it is a reliable metric for \emph{measurability} that accurately predicts when the detected signal contains evidence for precession. 




==> conclusion.tex <==
In most candidate astrophysical binary distributions, precession is likely to be first measured in a comparable-mass binary~\citep{Fairhurst:2019srr}.
We have considered a fiducial example of such a possible signal (mass-ratio $q=2$, \ac{snr} $\rho = 20$, and in-plane spin $\chi_p = 0.4$,
such that the precession contribution to the total \ac{snr} is $\rho_p = 5$), and performed an extensive parameter-estimation study that
has systematically explored the impact on parameter measurements of changes in each of the key source parameters:
the SNR, the in-plane spin magnitude, binary inclination, the binary mass ratio and aligned-spin contribution, the binary's total
mass, the polarisation, and sky location. These examples illustrate well-known features of precession signals~\citep{vecchio2004lisa, Lang:1900bz, Apostolatos:1994mx, Brown:2012gs, vitale2014measuring, abbott2017effects, Fairhurst:2019srr, berti2005estimating}, and
quantify their effect on both the measurement of precession, and their impact on the measurement accuracy and precision of
other parameters.

We have also verified that $\rho_p$ provides a suitable and intuitive metric for determining whether or not we have measured precession,
and shown that there is an approximate mapping between $\rho_p$ and the use of the Bayes factor to assess the evidence of precession.
We suggest that given these results, future large scale studies of precession can be made considerably computationally cheaper by
computing $\rho_p$, rather than a full Bayesian analysis.

We note that as $\rho_{p}$ captures precession by identifying additional power beyond a simple non-precessing waveform model, it could therefore be effected by phenomena such as eccentricity and higher order multipoles. As BFs simply compare the evidence for two models, one precessing and one non-precessing, using BFs as the sole metric would also be biased by properties like eccentricity and higher order multipoles. 

However, a similar approach to the 2-harmonic decomposition for precessing signals has recently been applied to
\acp{gw} including the effects of higher harmonics~\citep{mills2020measuring}.
In future work, we will combine these approaches and explore the measurability of precession
in systems with significant evidence for higher harmonics, and the impact of the combination of
higher modes and precession upon parameter accuracy. It may also be possible to account for eccentricity
through a similar decomposition.

The current study does not include higher harmonics, and uses a signal model (\texttt{IMRPhenomPv2}) that neglects two-spin precession effects,
mode asymmetries that lead to out-of-plane recoil~\cite{Kalaghatgi:2020gsq}, and detailed modelling of precession effects through merger
and ringdown. Although these effects are typically small, so is the imprint of precession on the signal, and it would be interesting in future to
investigate the impact of these additional features on our results. We also emphasize that, although we consider it to be extremely useful to
provide quantitative examples of the effects of each of the binary parameters, these will necessarily depend on the location in
parameter space of our fiducial example. However, having chosen a configuration from amongst what we expect to be the most likely
signals, we hope that these examples will act as a useful guide in interpreting precession measurements when they
arise in future gravitational-wave observations.


==> introduction.tex <==


In September 2015, the first direct detection of \acp{gw} marked the beginning of GW astronomy~\cite{Abbott:2016blz}.
Another 14 detections have been announced by the LIGO Scientific and Virgo collaborations (LVC),
the vast majority of which were due to \ac{bh} mergers~\citep{LIGOScientific:2018mvr, Abbott:2020uma, LIGOScientific:2020stg, Abbott:2020khf, Abbott:2020mjq, Abbott:2020tfl}.
Additional events have also been reported by independent groups~\citep{nitz20202, venumadhav2020new, zackay2019highly, zackay2019detecting}.
These GW observations have already provided significant insights into gravitational physics,
cosmology, astronomy, nuclear physics and fundamental physics (see e.g. Refs.~\cite{SchutzDeterminingHubbleconstant1986,Soares-Santos:2019irc, AbbottGravitationalWavesGammaRays2017,abbott2018gw170817,abbott2018gw170817stochastic,ligo2017gravitational,abbott2019tests,LIGOScientific:2018jsj}).
With an order of magnitude more observations expected over the next 5-10 years, as
the sensitivities of the LIGO~\cite{Aasi:2013wya, TheLIGOScientific:2014jea}, Virgo~\citep{acernese2014advanced} and KAGRA~\citep{aso2013interferometer} detectors improve and additional detectors come online,
GW astronomy from compact-binary mergers has the potential to transform our understanding of gravitational and
fundamental physics~\cite{Sathyaprakash:2019nnu,Bianchi:2018ula,Ford:2019nic}.

Everything we learn from GW \ac{bbh} observations is a consequence of a detailed
parameter estimation analysis that extracts the source parameters of the binary. While some parameters
are extracted with good precision, inspiral dominanted signals show strong correlations between certain parameters which means that they cannot
be measured so accurately, for example correlations between the binary's distance and inclination~\citep{Cutler:1994ys, LIGOScientificCollaborationandVirgoCollaborationPropertiesBinaryBlack2016, Usman:2018imj},
the two masses~\citep{Cutler:1994ys, Poisson:1995ef}, and the mass-ratio and spin components aligned to the binary's orbital angular
momentum~\citep{Poisson:1995ef, Baird:2012cu, farr2016parameter, ng2018gravitational}. As well as studies of the inspiral, work has been done to extract the source properties for high mass signals dominated by the merger ringdown, see e.g.~\cite{Graff:2015bba, Haster:2015cnn, Vitale:2016avz, Yu:2017zgi}.

Spin components misaligned with the binary's orbital angular momentum, leading to a precession of the binary's
orbital plane and hence modulations of the amplitude and phase, have not yet been unambiguously measured
in GW observations~\citep{LIGOScientific:2018mvr}, see Fig.~\ref{currentdetections}. Precession effects and correlations with other parameters are understood in
principle~\cite{Apostolatos:1994mx,Kidder:1995zr} but since theoretical signal models of precessing
binaries that include the merger and ringdown date from only shortly before the first detections~\cite{Hannam:2013oca,Pan:2013rra}, we have less experience of when precession will be measurable, and what the impact will be on other parameter measurements.

The purpose of this paper is to explore when precession will be measurable, and its impact on other parameter measurements, in
the kind of configurations that are representative of expectations from binary populations based on
LIGO-Virgo-KAGRA observations to date~\cite{LIGOScientific:2018mvr}. By utilizing the
precession \ac{snr}  $\rho_{p}$ ~\citep{Fairhurst:2019_2harm, Fairhurst:2019srr} as a
quantifier for the measurability of precession, we also verify that
$\rho_p$ is indeed a good metric for the measurability of precession across the vast majority of the
parameter space, and relate it to the standard means to identify the presence of
precession, the Bayes factor. In doing so, we show that computationally expensive parameter estimation runs can be avoided
by simply calculating the precession SNR.

\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.42]{current_detections_chi_p}
	\includegraphics[scale=0.42]{current_detections_rho_p}
	\caption{Plot showing the posterior distributions for $\chi_{p}$ and $\rho_{p}$ for all LIGO/Virgo \ac{bbh} observations. The $\chi_{p}$ posterior distribution (left hand side, colored) is compared to its prior (right hand side, white) in the form of a split violin plot. The $\rho_{p}$ posterior distribution is shown as a single violin. Horizontal grey lines show the 90\% symmetric credible interval. The solid black line shows the $\rho_{p} = 2.1$ threshold. Bounded \acp{kde}are used for estimating the probability density. Data obtained from the Gravitational Wave Open Science Center~\citep{abbott2019open}.}
	\label{currentdetections}
\end{figure*}

Previous work has explored the general phenomenology of precession effects: its increased
measurability with large in-plane spins~\citep{vecchio2004lisa, Lang:1900bz, Chatziioannou:2018wqx},
large mass ratios~\citep{vecchio2004lisa, Lang:1900bz},
high inclination~\citep{Apostolatos:1994mx, Brown:2012gs, vitale2014measuring, abbott2017effects, Fairhurst:2019srr, Vitale:2016avz},
and of course high SNR~\citep{vecchio2004lisa, Lang:1900bz, berti2005estimating}.
Beyond these general expectations, the \emph{quantitative} behaviour of parameter measurements in the presence of precession
has not been studied in great detail for typical LIGO-Virgo-KAGRA observations.
The measurability of precession for high mass ratio LIGO-Virgo-KAGRA observations like
GW190814 has been investigated in recent work~\cite{Pratten:2020igi}.

In this paper, we focus on the region of parameter space most likely to yield
binaries with observable precession: binaries of comparable mass, with moderate
in-plane and aligned-spin components ~\citep{Fairhurst:2019srr}.
We perform a series of one-dimensional investigations of the parameter space,
in which we vary one parameter at a time: total mass, mass ratio, spins
(both in-plane as characterized by $\chi_p$, and the aligned spin combination
$\chi_{\mathrm{eff}}$), the binary orientation (both the inclination of the orbit
and also binary polarization), and the sky location and show the impact of
varying each of the binary parameters individually.  These investigations serve
to confirm that much of the known phenomenology is apparent even at relatively low SNR, 
while also demonstrating that the
precession \ac{snr} can be effectively used across
a significant fraction of the parameter space to \textit{predict} the
observable consequences of precession \textit{without} the need for
computationally costly parameter estimation analyses.

This paper is structured as follows: Sec.~\ref{sec:precession} provides an introduction to precession, a brief recap of the two-harmonic
approximation that allows us to define $\rho_p$, and a summary of the importance of precession across the parameter space.
Sec.~\ref{sec:pe_standard} provides an introduction to the parameter estimation techniques used here, and parameter estimation results
and interpretation for our fiducial system.
In Sec.~\ref{sec:pe_results} we perform a series of one-dimensional explorations of the parameter space.
In Sec.~\ref{sec:rho_p_predict} we compare the predicted precession \ac{snr} with observations
and in Sec.~\ref{sec:bayes_factors} we compare precession \ac{snr} with the Bayes factors between precessing and non-precessing runs.
We conclude with a summary and discussion of future directions.


==> parameter_estimation.tex <==
We will adopt a parameter estimation methodology that uses matched filtering with phenomenological gravitational waveforms and Markov Chain Monte Carlo (MCMC) techniques to sample the posterior.
\par
We begin by introducing the matched filtering formalisation for parameter estimation. We assume that the time series received from the GW detectors can be decomposed as a sum of the GW signal, $h(t)$, plus noise, $n(t)$, which is assumed stationary and Gaussian with zero mean,
\begin{equation}
	d(t) = h(t) + n(t).
\end{equation}
%
Under the assumption of Gaussian noise, the probability of observing data $d$ given a signal $h(\bm{\lambda})$ parameterised by $\bm{\lambda} = \{\lambda_{1},\lambda_{2},...,\lambda_{N}\}$, otherwise known as the likelihood, is~\cite{finn1992detection},

\begin{equation} \label{eq:likelihood_calculation}
	p(d|\bm{\lambda}) \propto \exp\left(-\frac{1}{2}\langle d-h(\bm{\lambda}) | d - h(\bm{\lambda}) \rangle \right),
\end{equation}
%
where $\langle a | b \rangle$ denotes the inner product between two waveforms $a$ and $b$ and is defined as,
\begin{equation}\label{eq:inner_prod}
	\langle a | b \rangle = 4\text{Re}\int_{0}^{\infty}{ \frac{\tilde{a}(f)\tilde{b}^{*}(f)}{S_{n}(f)} df},
\end{equation}
%
where $S_{n}(f)$ is the one-sided power-spectral density (PSD) and $\tilde{a}$ denotes the Fourier transform of the gravitational waveform $a$.
\par
The posterior \ac{pdf} can then be computed through a simple application of Bayes' theorem,
\begin{equation} \label{bayesequation}
\begin{split}
	p(\bm{\lambda}|d) & = \frac{p(\bm{\lambda})p(d|\bm{\lambda})}{p(d)}, \\
	                & \propto p(\bm{\lambda}) \exp\left(-\frac{1}{2}\langle d-h(\bm{\lambda}) | d - h(\bm{\lambda}) \rangle \right),
\end{split}
\end{equation}
%
where $p(\bm{\lambda}|d)$ is the posterior distribution for the parameters $\lambda$, $p(\bm{\lambda})$ is the prior probability distribution where $\int{p(\bm{\lambda})d\bm{\lambda}}=1$, and $p(d)$ is the marginalised likelihood where $p(d)=\int{p(\lambda_{i})p(d|\lambda_{i})}d\lambda_{i}$. Posterior distributions for specific parameters can then be found by marginalising over all other parameters,
%
\begin{equation} \label{posteriorforoneparameter}
	p(\lambda_{i}|d) = \int{p(\boldsymbol{\lambda}|d) d\lambda_{1}...d\lambda_{i-1} d\lambda_{i+1}... d\lambda_{N}}.
\end{equation}

In the idealised situation of zero noise, Eq.~(\ref{eq:likelihood_calculation})
has a maximum at $h(\bm{\lambda})=h(\bm{\lambda}_{0})$. However, as can be seen in Eq.~(\ref{bayesequation}) the posterior also includes priors, this means that, as well as effects due to noise, certain priors may cause the
maxima to be deflected away from $h(\bm{\lambda})=h(\bm{\lambda}_{0})$. This would then lead to Eq.~(\ref{posteriorforoneparameter}) recovering a
biased posterior.


==> plot_explanation.tex <==
We now look at the effect of varying individual parameters one at a time on the recovered posteriors,
in particular focusing on the measurement of precession as described by the posterior distributions of
$\rho_p $ and $\chi_p$. All subsequent one-dimensional investigations of the parameter space maintain a 
constant \ac{snr} (except for Sec.\ref{ssec:snr} where the effect of the \ac{snr} is investigated). This is achieved by 
varying the distance to the source.

Primary results presented in this section will be displayed in the form of violin plots.
We show the $\chi_{p}$ posterior distribution (left hand side, colored) compared to the global prior (right hand 
side, white) unless otherwise stated. We show the $\rho_{p}$ posterior distribution as a single violin. Horizontal 
grey lines show the 90\% symmetric credible interval. Horizontal red lines show the simulated value. A solid 
black line corresponds to the $\rho_{p} = 2.1$ threshold. Bounded \acp{kde}are used for 
estimating the probability density. We use the same 2d contour plots and multi-dimensional corner plots as 
described in Sec.~\ref{sec:standard_pe}. Plots were generated with the PESummary~\cite{Hoy:2020vys} 
python package.


==> precession_theory.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.185]{precession_angles.png}
	\caption{Plot showing how the precession angles used in this study are defined in the co-precessing frame. The normal vector $\mathbf{\hat{n}}$ here indicates the line of sight of the observer, $\mathbf{\hat{L}}$ and $\mathbf{\hat{J}}$ are the orbital angular momentum and total angular momentum vectors respectively, $S_{1x}, S_{1y}$ and $S_{1z}$ are the x, y and z components of the spin on the larger black hole. Note that $\mathbf{J}, \mathbf{L}$ and $\mathbf{\hat{n}}$ are shown to be co-planar only for ease of illustration. It is not true in general.}
	\label{precession_angles}
\end{figure}

A binary consisting of two compact objects will slowly inspiral due to the emission of GWs.
Assuming that the binary is on a quasi-spherical orbit, it may be described by the
individual component masses, $m_{1}$ and $m_{2}$ (where we define $m_1 > m_2$ and we denote
the mass ratio to be $q = m_1/m_2 > 1$), and their spin angular momenta $\mathbf{S}_{1}$
and $\mathbf{S}_{2}$.
\par
For the case where the total spin is misaligned with the total orbital angular momentum,
$\mathbf{S}_{i} \times \mathbf{L} \neq 0$, the system undergoes
spin-induced precession.
In most cases $L \ll J$, and the system undergoes ``simple precession'', where the
orbital angular momentum precesses around the (approximately constant) total angular momentum,
$\mathbf{J} = \mathbf{S_{1}} + \mathbf{S_{2}} + \mathbf{L}$, and the spins precess such that
$\dot{\mathbf{S}} = - \dot{\mathbf{L}}$, where $\mathbf{S} = \mathbf{S_{1}} + \mathbf{S_{2}}$~\cite{Apostolatos:1994mx,Kidder:1995zr}.
\par
The strength of precession is characterised by the tilt angle of the binary's orbit, $\beta$,
defined as the polar angle between $\mathbf{L}$ and $\mathbf{J}$; see
Fig.~\ref{precession_angles}. $\beta$ is determined primarily by the total spin in the plane, and
the binary's mass ratio and separation. At leading order the magnitude of the binary's orbital angular
momentum is given by $L = \mu \sqrt{Mr}$, and we can write,
%
\begin{equation} \label{eq:opening_angle}
	\cos \beta = \frac{\mu\sqrt{M r} + S_{\parallel}}{\left[\left(\mu\sqrt{M r} + S_{\parallel}\right)^{2} + S_{\perp}^{2} \right]^{1/2}},
\end{equation}
%
where $M = m_{1} + m_{2}$ is the total mass of the source, $\mu = m_{1}m_{2}/ M $ is the reduced
mass, $r$ is the separation and
$S_{\parallel}$ and $S_{\perp}$ are the total spin parallel and perpendicular to $L$ respectively.
In general, the larger the ``opening angle'', $\beta$, the more prominent the precession effects.

In simple precession cases, $\beta$
slowly increases during inspiral. This temporal variation is mostly dependent on the variation of r as,
 throughout the portion of the binary's inspiral that is visible in the GW detectors, 
 $ \mu, M, S_{\parallel} $ and $ S_{\perp}$ are all approximately constant.
 Therefore, $\beta$ also typically varies very little over the duration that is visible in the GW detectors, 
 and it is possible to make the simplifying assumption that $\beta$ remains constant.
This assumption has been used to good effect in previous work, e.g., Ref.~\cite{Brown:2012gs}, although in this work we make
no assumptions about $\beta$.

It is often convenient to quantify the binary's in-plane spin by the scalar quantity $\chi_{p}$~\cite{Schmidt:2014iyl} (see Refs.~\cite{Gerosa:2020aiw, Thomas:2020uqj} for 
 alternative measures).
$\chi_{p}$ estimates a time-average of the in-plane spin components that drive precession, motivated by the leading-order PN precession
equations~\cite{Apostolatos:1994mx,Kidder:1995zr}, and is defined as,
%
\begin{equation} \label{chi_p}
	\chi_{\text{p}} = \frac{1}{A_{1}}\text{max}\left(A_{1}S_{1\perp},A_{2}S_{2\perp}\right),
\end{equation}
%
where $A_{1} = 2+3q/2$ and $A_{2} = 2+3/(2q)$ and $\mathbf{S}_{i\perp}$ is the component of the spin
perpendicular to $\mathbf{L}$ on the $i$th black hole. $\chi_{p}$ as defined above, 
 takes values between $0$ (non-precessing system) and
 $+1$ (maximally precessing system).

\subsection{Two harmonic approximation}
\label{ssec:two_harm}

Non-zero values of $\beta$ and $\chi_p$ indicate that a binary is precessing, and, if all other parameters are kept constant,
they parameterise the amount of precession in a system. However, they are not sufficient to tell us whether precession will
be \emph{observable}. Precession appears in the signal as modulations of the amplitude and phase, but these also depend on the
binary orientation and signal polarisation. Refs~\citep{Fairhurst:2019_2harm, Fairhurst:2019srr} introduce a
method for decomposing a precessing waveform into a series of five {\it{non-precessing harmonics}}, where the
characteristic modulations of a precessing signal are caused by the beating of these {\it{harmonics}}.
The harmonics form a power series in the parameter,
%
\begin{equation}
b = \tan(\beta/2).
\end{equation}
%
In most regions of parameter space, the two leading harmonics (a leading-order term independent of $b$, and a first-order
term proportional to $b$)
are sufficient to capture the significant precession features in the waveform, and the other harmonics
can be neglected. As discussed in detail in Sec.~V of Ref.~\cite{Fairhurst:2019_2harm}), 
these other precession harmonics can be ignored for binaries where $\beta \lesssim 45 \degree$.
In general this is true for all binaries, apart from relatively extreme systems, for example, those that have $\theta_{JN}$ close to 
edge-on \emph{and} are either highly precessing or have very large negative spins. 
 
  Thus, for almost all signals we expect to observe, the waveform can faithfully be expressed as,
%
\begin{equation}\label{eq:h_2harm}
	h(f) \approx \mathcal{A}_{0} h^{0}(f) + \mathcal{A}_{1} h^{1}(f) \, ,
\end{equation}
%
where $\mathcal{A}_{0}$ and $\mathcal{A}_{1}$ are complex, orientation dependent amplitudes, and $h^{0}(f)$ and $h^{1}(f)$
are the waveforms of the two leading harmonics.  For a detector with a one-sided noise spectral density of $S_n(f)$, the relative amplitude
of the harmonics is given by
%
\begin{equation}\label{eq:b_bar}
\overline{b} := \frac{ |h^{1} | }{ | h^{0} |} = \sqrt{\frac{\int df \frac{ |h_{1}(f)|^{2}}{S_{n}(f)}}{\int df \frac{ |h_{0}(f)|^{2}}{S_{n}(f)}}} \, .
\end{equation}
%
which is the average value of $b$ over the observable signal, weighted by the signal strength in the detector.
The complex amplitudes $\mathcal{A}_{0,1}$ depend upon the extrinsic parameters of the binary:
the distance $d_L$, angle between $\mathbf{J}$ and the line of sight $\mathbf{\hat{n}}$, polarization angle $\psi$, reference phase $\phi_0$,
and the reference precession phase $\phi_{JL}$\footnote{This is equivalent to $\alpha_{0}$ in Ref.~\citep{Fairhurst:2019_2harm}}.
It is convenient to introduce a reference distance $d_{0}$, which is incorporated into the definitions of the harmonics $h_{0}$ and $h_{1}$.
The amplitudes are then defined as,%
%
\footnote{These expressions are equivalent to Eq.~(33) in \cite{Fairhurst:2019_2harm}, which are restricted to the
special case where $F_{+} = \cos 2\psi$ and $F_{\times} = -\sin 2\psi$.  More generally, the detector
response also depends upon the sky location in addition to the polarization.}
%
%
\begin{align}\label{eq:2harm_amps}
	\mathcal{A}_{0} =& \frac{d_0}{d_L} \left[F_{+} \left(\frac{1+\cos^2 \theta_{\rm JN}}{2} \right) + i F_{\times}\cos \theta_{\rm JN} \right] \times \nonumber \\
	& e^{-i  (2 \phi_{o} + 2 \phi_{JL} )}, \nonumber \\
	\mathcal{A}_{1} =&\frac{d_0}{d_L}  \left[F_{+} \sin 2\theta_{\rm JN}  + 2 i F_{\times} \sin \theta_{\rm JN}  \right] \times \nonumber \\
	& e^{-i (2 \phi_{o} + \phi_{JL} )}.
\end{align}
%
The relative significance of the two harmonics is encoded by
\begin{eqnarray}\label{eq:zeta}
	\zeta & := & \frac{\overline{b} \mathcal{A}_{1}}{\mathcal{A}_{0}} \\
	& = & \overline{b} e^{i \phi_{JL}}  \, \left(\frac{
	F_{+} \sin2\theta_{\rm JN}  + 2 i F_{\times} \sin \theta_{\rm JN}  }{
	\tfrac{1}{2} F_{+} (1 +\cos^2 \theta_{\rm JN})  + i F_{\times} \cos \theta_{\rm JN}  }\right)  \, , \nonumber
\end{eqnarray}
%
where the detector response $F_{+, \times}$ is calculated using the polarization angle appropriate for a co-ordinate system defined with the z-axis
along the direction of total angular momentum $\mathbf{J}$.

The observability of precession can then be characterised by the precession \ac{snr} $\rho_{p}$,
defined as the \ac{snr} in the weaker of the two harmonics, and also expressible as a fraction of $\rho = |h|$, the total signal
SNR,
%

\begin{eqnarray}\label{rho_p}
	\rho_{p} &=& \mathrm{Min}{\left(|\mathcal{A}_{0}h^{0}|, |\mathcal{A}_{1}h^{1}|\right)} \nonumber \\
	&=&  \rho \, \left(\frac{ \mathrm{min}(1, |\zeta| )}{ \sqrt{1 + |\zeta|^{2}}}\right).
\end{eqnarray}

Eq.~\ref{rho_p} assumes that the two harmonics are orthogonal. If the two harmonics are not orthogonal, such that the overlap between the two harmonics is non-zero, it is necessary to consider only the orthogonal part of
the less significant harmonic when calculating the precession SNR. This introduces additional overlap terms in Eq.~\ref{rho_p}, see Ref.~\cite{Fairhurst:2019_2harm} for details.  Despite the fact that the majority of cases
considered in this paper have a small overlap between the two harmonics (less than 10\%), we use the
full form of $\rho_{p}$ as defined in Ref.~\cite{Fairhurst:2019_2harm}. At
higher masses, the two harmonics have significant overlap and we discuss the impact of this when we vary the total mass of the binary below.

The quantity $ \rho_p$ parameterises the \emph{observable} precession,
it is therefore the \emph{measured} quantity in the data.
By considering what we actually measure in the data we are able
to understand many of the correlations and degeneracies in the physical
parameters that are \emph{caused} by the presence of (or lack of)
measurable precession.

In the absence of precession,
$\rho_{p}^{2}$ will be $\chi^{2}$ distributed with two degrees of freedom. Consequently,
 if there is no observable precession in the system, $\rho_{p} \geq 2.1$ in only 10\% of cases. Thus far we have
used $\rho_{p} = 2.1$ as a simple threshold to determine if there is any observable precession in the system.
We revisit this in more detail in Sec.~\ref{ssec:predict_np}.


\subsection{Observability of precession}
\label{ssec:rho_p}

The strength of the modulations in the GW signal depend primarily on the opening angle, $\beta$, and this is reflected in the expansion
parameter $b$ in the two-harmonic approximation; the precession frequency $\dot{\alpha}$ also plays a role.
The strength of the modulations in the \emph{observed} signal also depend on the binary's inclination to the observer, $\theta_{\mathrm{JN}}$, and the
detector polarisation $\psi$, and these are all incorporated into the precession \ac{snr} $\rho_p$, through Eqs.~(\ref{eq:zeta}) and
(\ref{rho_p}). From these we can draw immediate
conclusions about the scenarios in which precession will be most easily measured. These observations are in general not new (see, as always,
the pioneering discussions in Refs.~\cite{Apostolatos:1994mx, Kidder:1995zr}), but we summarise
them here and, where salient, present them in terms of the two harmonic formalism, which highlights the insights and intuition that are
simplified in this formulation. We then compare these expectations with the quantitative results that we find in our full parameter estimation
study.

Our first basic picture of the strength of precession effects comes from Eq.~(\ref{eq:opening_angle}), which gives the dominant
effect on $\beta$ during
the inspiral. If we first consider cases where the spin is entirely in the orbital plane, i.e., $S_{||} = 0$, we see that the opening angle $\beta$ will
be zero if $S_\perp = 0$ (as we would expect), and increases linearly for small $S_\perp$. The opening angle also increases as
$\mu$ decreases, i.e., as the mass ratio is increased. Eq.~(\ref{eq:opening_angle}) is no longer accurate near merger, and for
 equal-mass systems $\beta$ does not become large, but for large mass ratios the opening angle can approach $90^{\circ}$.

If we now consider non-zero $S_{||}$, we see that the level of precession will be reduced for systems with a positive aligned-spin
component, and will be increased for systems with a negative aligned-spin component. The importance of this effect will depend on
the other terms, but we can see that for a high-mass-ratio system where $\mu$ is very small, and close to merger, so $rM$ is also small,
the aligned-spin component will have a strong effect on $\beta$, and therefore the measurability of precession. A negative $S_{||}$ is
necessary to achieve $\beta > 90^{\circ}$, and for large mass-ratio systems near merger (small $\mu$ and $r M$) and large negative
$S_{||}$, $\beta$ can approach $180^{\circ}$, but such systems will be rare.

The measurability of precession also depends on the orientation of the binary with respect to the detector, $\theta_{\mathrm{JN}}$.
As we see in Eq.~(\ref{eq:zeta}), precession effects will be minimal if $\theta_{\mathrm{JN}}\sim 0^{\circ}$ or $180^{\circ}$,
i.e., the observer views the system from the direction of $\mathbf{\hat{J}}$.  We expect precession to be strongest in the observed waveform for orientations close to $\theta_{\mathrm{JN}} \sim 90^{\circ}$.
Additionally, when the detector, or network is primarily sensitive to the $\times$ polarization, precession effects will be more significant.
The amplitude of the $k=1$ harmonic vanishes in the $+$ polarization for both face on $\theta_{\mathrm{JN}}= 0^{\circ}$ and $180^{\circ}$ and edge-on $\theta_{\mathrm{JN}} = 90^{\circ}$ systems,
while the $\times$ polarization is maximal for edge-on systems.  Additionally, the $\times$ polarization for the $k=0$ harmonic vanishes
for edge on systems, while the $+$ polarization is only reduced by a factor of two.  Thus, even when $b$ is small, there can be observable
precession when the system is close to edge on and the network is preferentially sensitive to the $\times$ polarization. For a given
choice of masses and spins, the maximum precession \ac{snr} is $\rho_p = \rho / \sqrt{2}$.


==> results_bayesfactor.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{BF_vs_rho_p}
	\caption{
	Plot comparing the Bayes factor in favour of precession to the inferred $\rho_{p}$
	distribution. Bayes factors were calculated by comparing the evidences for a precessing analysis
	and a non-precessing analysis. The uncertainties on the Bayes factors are calculated by taking the
	$90\%$ confidence interval across multiple {\sc{LALInferenceNest}} chains. The solid line uses
	the median of the $\rho_{p}$ distribution. The shading gives the $1\sigma$ and $2\sigma$ uncertainties
	on the $\rho_{p}$ measurement. The solid black lines shows the $\rho_{p} = 2.1$ threshold.}
	\label{fig:rho_p_vs_bayesfactor}
\end{figure}

An alternative method for identifying evidence for precession can be calculated within the
Bayesian framework. We can calculate the Bayes factor, $\mathcal{B}$, by comparing the
marginalized likelihoods (see Eq.~(\ref{bayesequation})) from two competing
hypotheses (A, B)~\citep{jaynes2003probability},
%
\begin{equation}
	\ln{\mathcal{B}} = \ln{p(d_{A})} - \ln{p(d_{B})}.
\end{equation}
%
Bayes factors have thus far been the gold standard
for identifying evidence for precession within the GW community and have been used
extensively in previous works, see e.g., Ref.~\cite{Pratten:2020igi}.

In the same way that Bayes factors can be used to quantify evidence for precession, it is also possible to
quantify the significance of a GW signal by calculating the Bayes factor for signal verses
noise~\citep{Veitch:2009hd}. It has been shown that the log Bayes factor for signal versus noise scales
approximately with $\rho^2$~\citep{cornish2011gravitational}. Here, we investigate
the relationship between the Bayes factor in favour of precession and the precession \ac{snr} $\rho_{p}$.
Both of  these quantities have been used together in recent works when assessing the evidence for
observable precession~\citep{LIGOScientific:2020stg, Abbott:2020khf, Pratten:2020igi}

For a subset of the runs described in Section.~\ref{ssec:inclination}, we reran the analysis
using the aligned-spin waveform model {\texttt{IMRPhenomD}}. Bayes factors in favour
of precession could then be calculated and compared to the derived $\rho_{p}$ posterior
distributions.

Fig.~\ref{fig:rho_p_vs_bayesfactor} shows an approximately linear relationship between the
log Bayes factor ($\ln \mathrm{BF}$) and the square of the precession \ac{snr} ($\rho_{p}^{2}$).
This is expected given that the likelihoods recovered from the precessing waveform model will be
larger than the likelihoods recovered from the aligned-spin waveform model
by a factor of $\exp(\rho_{p}^{2} / 2)$.

The commonly used heuristic when assessing the strength of evidence using Bayes factors is that
 $ 1 \leq \ln\mathrm{BF} \geq 3 $ is marginal evidence and $\ln\mathrm{BF} > 3 $  is strong evidence in favour of a hypothesis.
From the plots above we conclude that if 90\% (50\%) of the $\rho_{p}$ posterior distribution is above the $\rho_{p}=2.1$ threshold, this corresponds to a $\ln\mathrm{BF} \approx 3.5$ ($\ln\mathrm{BF} \approx 0.8$) and is therefore very strong (marginal)
evidence for precession. The posterior distribution on $\rho_{p}$ can therefore
be approximately mapped to the commonly used $\ln\mathrm{BF}$. Assessing the strength of evidence for precession using $\rho_p$ would also reduce the need for additional parameter estimation runs using non-precessing models, which are \emph{necessary} to compute the Bayes factor. This reduction in computational
cost will not be significant for a single event, but for population analyses and large scale PE studies this
alternative metric could be extremely useful.

==> results_chi_eff.tex <==
\begin{figure*}[t]
        \centering
        \includegraphics[scale=0.4]{mass_ratio_chi_p}
        \includegraphics[scale=0.4]{mass_ratio_rho_p}
        \caption{ Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior (left) and $\rho_p$ (right). Distributions are plotted for varying mass ratio. Parameters other than the mass ratio of the signal match the ``standard injection'' (see Table~\ref{tab:standard_run}).}
        \label{chi_p_vs_mass_ratio}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.4]{chi_eff_chi_p}
	\includegraphics[scale=0.4]{chi_eff_rho_p}
	\caption{ Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior conditioned on the $\chi_{\mathrm{eff}}$ and mass ratio posterior distributions (left) and $\rho_p$ (right). Distributions are plotted for varying $\chi_{\mathrm{eff}}$. Parameters other than the $\chi_{\mathrm{eff}}$ of the signal match the ``standard injection'' (see Table~\ref{tab:standard_run}).}
	\label{chi_p_vs_chi_eff}
\end{figure*}

%When the mass ratio of the binary increases, the large black hole's spin contributes more significantly to the total angular momentum,
%as can be seen in Eq.~(\ref{eq:opening_angle}), and the opening angle $\beta$ (and as a result $b$) increases.  Thus, a system with a larger mass
%ratio will have more observable precession than to an equal-mass system.

Fig.~\ref{chi_p_vs_mass_ratio} shows how the inferred precessing spin and precession \ac{snr} varies with the mass ratio of the system.  As expected
from the general considerations presented in Sec.~\ref{sec:precession}, as the mass ratio increases, an in-plane spin on the larger \ac{bh}
leads to a larger opening angle and more significant precession effects.
For near equal-mass systems
($q \lesssim 1.5$), the inferred $\chi_{p}$ posterior distribution resembles its prior, and there is not significant power in precession, as shown by the value of $\rho_{p}$.
As the mass ratio increases, the inferred power in precession also increases and for $q \gtrsim 2.5$, the 90\% credible interval of the
inferred $\rho_{p}$ distribution is entirely above $\rho_{p} = 2.1$.  At this stage, precession is clearly identified and $\chi_{p} \approx 0$
is clearly excluded.  In addition, the maximum value of $\chi_p$ is also bounded away from maximal.

Fig.~\ref{chi_p_vs_chi_eff} shows how varying $\chi_{\mathrm{eff}}$ affects our ability to measure precession.
A system with a large negative $\chi_{\mathrm{eff}}$ results in a larger
opening angle compared to an equivalent system with a large positive $\chi_{\mathrm{eff}}$.  Thus, based upon
Eq.~(\ref{eq:opening_angle}), we expect the observable impact of precession to be greater for negative values of
$\chi_{\mathrm{eff}}$ and smaller for positive values.  The results are consistent with this expectation, in that the precession SNR
decreases with increasing $\chi_{\mathrm{eff}}$ and the width of the recovered $\chi_p$ distribution increases.
However, for the $\chi_{\mathrm{eff}} = 0.4$ analysis, we find that the range of $\chi_{p}$ is restricted, with
both $\chi_{p} = 0$ and $\chi_{p} = 1$ excluded.  This is \textit{not} due to the measurement of precession, but
is actually due to the measured non-zero aligned-spin component.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.47\textwidth]{a_1_tilt_1_conditioned_prior}
	\caption{2d contours showing the prior 90\% credible interval over the primary spin magnitude and
	spin direction parameter space. Blue shows the global prior and red shows the global prior
	conditioned on the $\chi_{\mathrm{eff}} = 0.4$ mass ratio and $\chi_{\mathrm{eff}}$ posterior
	distributions}
	\label{fig:conditioned_prior}
\end{figure}

A non-zero measurement of $\chi_{\mathrm{eff}}$ forces $\chi_{p} < 1$ as the primary and
secondary spin magnitudes must be less than unity. For example, in the $\chi_{\mathrm{eff}} = 0.4$ analysis, we measure
$\chi_{\mathrm{eff}} = 0.38^{+0.07}_{-0.07}$. Under the single spin assumption, this limits
$\chi_{p} < 0.95$. Similarly, since we are using prior distributions that are uniform in spin magnitude
and orientation, the observation of a large aligned spin component leads to greater support for a large in-plane
spin component.  This is shown in Fig.~\ref{fig:conditioned_prior}, where we plot both the uninformed prior on the
primary spin as well as the prior conditioned on $\chi_{\mathrm{eff}} = 0.4$, which removes all support for $\chi_p \approx 0$.

The $\chi_{p}$ measurement for the $\chi_{\mathrm{eff}}=0.27$ and $0.4$ analyses are similar to the conditional prior
but do restrict the lower $\chi_{p}$ bound beyond prior effects.  Although the distribution for $\rho_p$ does extend to zero,
it still peaks above $\rho_p = 2.1$ indicating some evidence, although not particularly strong, for precession.

As we vary the mass ratio and aligned spin, the length of the waveform will change.  In particular, the
aligned spin and high mass ratio configurations produce longer waveforms than those with anti-aligned spins and
equal masses~\citep{Campanelli:2006uy}.  In principle, this will impact the measurability of precession, as
longer waveforms allow for a greater number of precession cycles in the detectors' sensitive band.
For very short signals, with less than one precession cycle in band, the two leading harmonics are no longer orthogonal
(or even approximately so), which make it more challenging to unambiguously identify the second harmonic.  This is not
an issue for the signals considered here, but does become important when we vary the mass of the binary in Section \ref{ssec:total_mass}.
With a greater number of precession cycles, we will also be able to more accurately measure the precession frequency (the frequency
difference between the harmonics), which may improve the measurement of mass ratio \cite{OShaughnessy:2014shr}.
However, it is still the precession \ac{snr} that determines the observability of precession.
Finally, we note that changing the mass ratio and aligned spin will change the overall amplitude of the waveform.
Since our study is performed at a \textit{fixed SNR}, this simply leads to the signals being placed at a larger or smaller distance and
therefore doesn't impact the results presented here.


%The power orthogonal to the dominant harmonic is somewhat related
% to the number of precession cycles. If there is less than one precession cycle in band then the two harmonics are very close
% to parallel, thereby considerably reducing the orthogonal power. As the number of precession cycles grows (i.e. above 1 or 2 cycles in band),
% we do not expect the number of precession cycles to substantially increase $\rho_{p}$. Consequently,
% despite a more positive $\chi_{\mathrm{eff}}$ resulting in a longer waveform~, and therefore more precession
% cycles, a system with a
%large negative $\chi_{\mathrm{eff}}$ will have more observable precession compared to a system with a
%more positive $\chi_{\mathrm{eff}}$. Consequently, for the same amount of measurable precession, a system
%with a large positive $\chi_{\mathrm{eff}}$ requires a larger $\chi_{p}$ to produce a comparable opening
%angle.


==> results_chi_p.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.4]{chi_p_and_chi_p_prior.pdf}
	\includegraphics[scale=0.4]{chi_p_rho_p.pdf}
	\caption{Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior (left) and $\rho_p$ (right). Distributions are plotted for varying $\chi_{p}$. Parameters other than $\chi_{p}$ match the ``standard injection'' (see Table~\ref{tab:standard_run})}
	\label{fig:chi_p_vs_chi_p}
\end{figure*}

We now look at the effect of varying the amount of precession in the system,  varying $\chi_p$
from 0 to 1 in steps of 0.25. At $\chi_{p} = 1$ we have maximal spin, all in the plane of the binary.
The inferred values of precessing spin and precession \ac{snr} are shown in Fig.~\ref{fig:chi_p_vs_chi_p}.
We observe, as expected, that increasing the in-plane spin leads to an increase in
the magnitude of precession effects observable in the system. With zero precessing spin, there
is no evidence for precession in the system; the recovered $\chi_p$ is consistent with zero%
%
\footnote{We do not expect the $\chi_p$ posterior to contain $\chi_p = 0$ as there is no prior support there, however the posterior is relatively well constrained at low precession.}.
Similarly, there is no support for significant precession SNR, with $\rho_p$ constrained near zero.
%
As $\chi_p$ increases, the amount of precession in the system grows and the measurement of $\chi_p$ becomes both more accurate and more precise.
Fig.~\ref{fig:chi_p_vs_chi_p} shows the relationship between $\rho_p$ and $\chi_p$, and a larger value for $\rho_p$ enables a better measurement for $\chi_p$.



\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.4]{chi_p_2d_contour_plot_mass_ratio_and_chi_eff}
	\includegraphics[scale=0.4]{chi_p_2d_contour_plot_theta_jn_and_luminosity_distance}
	\caption{Two dimensional posteriors for (left) mass ratio and aligned spin, $\chi_{\mathrm{eff}}$, (right) binary orientation and distance. Contours show the 90\% confidence interval. Bounded two-dimensional KDEs are used for estimating the joint probability density. The black circle with corresponding horizontal and vertical lines indicates the simulated values. For the simulated distance, a solid horizontal band indicates the maximum and minimum simulated values.
	}
	\label{fig:chi_p_insight_contours}
\end{figure*}

Fig.~\ref{fig:chi_p_insight_contours} shows how the inferred mass ratio--aligned spin and
distance--orientation contours change as the magnitude of the in-plane spins change.  When
there is no observable precession in the system, there is a clear degeneracy in both cases.
However, as precession effects become stronger the degeneracy between both pairs of
parameters is broken.  If $\rho_p$ is small then this can be explained by both a small amount of
precession observed at almost any inclination angle, or a large $\chi_p$ observed close to face on, as seen in
Fig.~\ref{fig:rho_p_chi_p}.  Since precession effects are not strong enough
to provide an accurate measurement of the orientation, the degeneracy between distance and $\theta_{JN}$ persists.
When $\rho_p$ clearly excludes small values, there is \emph{no support} for close to face-on signals, allowing a more precise measurement
of the inclination angle $\theta_{JN}$, breaking the degeneracy with distance.

Stronger precession also allows for improved measurement of the mass ratio.  The opening angle $\beta$, and consequently the
precession parameter $\bar{b}$, increases as the mass-ratio is increased, as can be seen
from Eq.~(\ref{eq:opening_angle}).
Thus, when strong precession effects are observed,
the signal is inconsistent with an equal mass system.  In addition, the difference in
frequency between the two leading precession harmonics depends upon the mass-ratio \cite{Fairhurst:2019_2harm}, and
this may also improve our measurement of $q$. This can also be seen from the precession dynamics,
where the precession rate of $L$ around $J$, $\dot{\alpha}$, depends the mass ratio, and
the number of observable precession cycles corresponds to improved accuracy in the measurement of the
mass ratio~\cite{OShaughnessy:2014shr}.

As $\chi_p$ is increased, the peak of the recovered $\rho_p$ distribution is closer to
the simulated value.  This is likely due to a better
measurement of the binary orientation as shown in Fig. \ref{fig:chi_p_insight_contours}.


==> results_mass_ratio.tex <==
\begin{comment}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{mass_ratio_violin_chi_p.png}
	\includegraphics[width=0.4\textwidth]{mass_ratio_violin_rho_p.png}
	\caption{Observability of precession for varying mass ratio.  Violin plots showing the recovered posterior distributions distributions for $\chi_p$ (left) and $\rho_p$ (right).  The mass ratio is varied between equal mass, $q=1$, and a mass ratio of 4:1.  The other parameters of the signal remain unchanged, in particular $M =  40 M_{\odot}$, $\chi_{\mathrm{p}}=0.4$, $\rho = 20$ and $\theta_{JN} = 60 \degree$. }
	\label{chi_p_vs_q}
\end{figure*}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{mass_ratio_2d_mass_ratio_chi_eff}
	\caption{Accuracy of recovery of mass ratio and spin for a series of simulated signals.  }
	\label{mass_ratio_spin}
\end{figure}

As the mass ratio of the binary increases (away from equal mass, $q=1$), the relative contribution of the large black hole's spin to the 
total angular momentum of the system increases.  This leads to an increase in the opening angle $\beta$, as can be seen from Eq.~(\ref{eq:opening_angle}), leading to an increase in the amount of precession.  Additionally, as the mass ratio increases, the relative contribution of the second harmonic will increase, leading to greater observational signatures of precession in the waveform.


In Sec.~\ref{} we saw that the other parameter that strong affects the measurability of precession is the mass ratio. 
In this section, we inject waveforms with total mass $M=30M_{\odot}$, zero aligned spins, $\chi_{\text{p}}=0.75$, viewed at an inclination 
angle of $\pi/3 \text{rad}$. We allow the mass ratio to vary between $1\leq q \leq 4$ in steps of $0.25$. \mdh{The plot does not have this many
mass ratios!!}. To demonstrate that for higher mass ratios precession can be measured even at low SNRs, we consider an \ac{snr} of 
$\rho = 13$. 
Fig. \ref{chi_p_vs_q} demonstrates the strong relationship between the mass ratio and the measurability of precession with an increase in 
mass ratio decreasing the 90\% confidence region of the $\chi_{p}$ posterior. As we saw earlier, this can be explained by returning to the 
definition of the opening angle, Eq.~\ref{opening_angle}. We see that the opening angle is dependent on the mass ratio through the 
reduced mass $\mu$, with an increase in the mass ratio leading to an increase in the opening angle. This therefore increases the amount of 
precession in the system, making it easier to measure.
\par
Once again, this description matches the posterior PDFs of $\rho_{p}$ with larger mass ratios leading to support for larger $\rho_{p}$. 
We find that except for equal mass, there is no support for $\rho_{p}$ within our ROPE and therefore we can say with certainty that we 
have measured precession for all cases with $q >1$. 
\par
Interestingly, we find that extremal $\chi_{p}$ is only excluded for $q>2$. We suspect that this is because... \mdh{Is it? Also, why does the 
peak of $\chi_p$ overshoot the correct value for $q=4$?} 
\par
We observe a bias for $q=3$ where the posterior \ac{pdf} peaks away from the injected value. This is because the $\chi_{\text{eff}}$ \ac{pdf} shows support for negative aligned spins with $\chi_{\text{eff}} = 0$ lying outside of the 90\% confidence region. The reason for this is because the true value of the smaller mass lies outside of the prior bounds. Consequently, in order to recover the true chirp mass, the mass ratio must be increased and $\chi_{\text{eff}}$ decreased to compensate. \mdh{Looking at the plot, $q=3$ is fine, but $q=4$ is off. ??} 
\end{comment}


==> results_orientation.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.4]{inc_and_chi_p_prior.pdf}
	\includegraphics[scale=0.4]{inc_rho_p.pdf}
	  \caption{Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior (left) and $\rho_p$ (right). Distributions are plotted for varying  $\theta_{JN}$. Parameters other than $\theta_{JN}$ match the ``standard injection'' (see Table~\ref{tab:standard_run})}
	\label{chi_p_vs_thetaJN}
\end{figure*}

It is well known that the inclination angle will
affect our ability to measure precession, as outlined in the discussion in Sec.~\ref{sec:precession}.
In particular, from Eq.~(\ref{eq:zeta}) we see that in the two-harmonic approximation the second harmonic vanishes when $\theta_{\rm{JN}} = 0^{\circ}$ or $180^{\circ}.$
In this section we consider the effect of changing the orientation of our standard configuration, which allows
us to quantify how it will manifest in realistic LIGO-Virgo signals. A related study has looked at the effect at higher
mass ratios~\cite{Pratten:2020igi}.

The effect of varying $\theta_{\rm{JN}}$ is shown in Fig.~\ref{chi_p_vs_thetaJN}.
For binaries where the total angular momentum is nearly aligned with the line of sight, 
precession effects are not observable, as is clear from both the $\rho_p $ and $\chi_p$ posteriors.  It is not until $\theta_{JN} \ge 40\degree $ that we begin to be able to measure precession.  Although the accuracy of the measurement clearly improves as we increase $\theta_{JN}$, the uncertainty in the measurement of $\chi_{p}$ remains large and even at $\theta_{JN} = 90\degree$ the posterior is very broad.  This can be understood by considering the degeneracies shown in Fig.~\ref{fig:rho_p_chi_p} for the standard signal and in Fig.~\ref{fig:inc_rho_p_chi_p_contour} for the $\theta_{JN} = 90^{\circ}$ signal.  In both cases, the measured quantity, $\rho_p$, is relatively well constrained but neither the binary orientation nor $\chi_p$ are accurately measured.  The observed precession is consistent with both a highly inclined system with lower precessing spin (i.e., low $\chi_p$ and large $\theta_{JN}$) or by a less inclined system with higher precessing spin (i.e., high $\chi_p$ and small $\theta_{JN}$).   Both of these will produce similar observable effects in the waveform.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.47\textwidth]{inc_chi_p_rho_p_countour}
	  \caption{A corner plot showing the recovered values of binary orientation $\theta_{JN}$, precessing spin $\chi_{p}$ and precession \ac{snr} $\rho_{p}$ for a system simulated at edge on. Shading shows the $1\sigma$, $3\sigma$ and $5\sigma$ confidence intervals. Black dots show the simulated values, We see the strong correlation between $\theta_{JN}$ and $\chi_{p}$ reflecting the measurement of a certain $\rho_{p}$  }
	\label{fig:inc_rho_p_chi_p_contour}
\end{figure}

This allows us to explain the measured posterior for $\chi_p$. At low inclination the posterior is consistent with small values of $\chi_p$.  While we are unable to rule out large $\chi_p$, there is limited support as it would require the system to be observed very close to face-on, otherwise precession effects become significant.  At large values of $\theta_{JN}$, when precession is clearly observable in the signal, $\chi_p = 0$ is excluded but the distribution remains broad and extends to $\chi_p = 1$.


==> results_prediction.tex <==
For the majority of simulations presented in this paper, the recovered
distribution for the precession SNR, $\rho_{p}$, has been peaked
significantly below the simulated value, although in nearly every case the
simulated value does lie within the $90\%$ confidence region.  While the
naive expectation is that the recovered posterior will peak at the simulated
value, for complex parameter recovery where there are dependencies and
degeneracies between the different parameters, this is often not the case.
We have already seen that the distance is typically over-estimated in the
simulations we have performed --- this is a well-known effect and arises for
two reasons, first that the network is less sensitive to sources from the chosen
sky location than from other locations consistent with the observed signal (as
discussed in Sec.~\ref{ssec:sky_loc}), and second that the signal
was simulated significantly inclined from face-on, yet preferentially recovered
close to face-on (as discussed in Sec.~\ref{ssec:inclination}).
Similarly, it seems likely that the signals we have
simulated have more significant precession effects (deliberately, as we wish
to understand the observability of precession) than the vast majority of
possible sources.  Thus, our conjecture is that there is a much larger volume of parameter space
consistent with low $\rho_{p}$ and this will bias the recovered value to be
smaller than the simulated one.

In order to test this hypothesis, we would like to
\textit{predict} the
distribution of the precessing SNR $\rho_{p}$ based upon the simulated value and
information gleaned from a non-precessing analysis.
We take advantage of the fact that that in the two-harmonic approximation,
the likelihood in Eq.~(\ref{likelihood_calculation}) can be factorized into two terms:
a non-precessing cmponent (dependent on $h_{0}$) $\Lambda_{\mathrm{np}}(\mathbf{\lambda})$
 and precessing component (dependent on $h_{1}$) $\Lambda_{\mathrm{p}}(\mathbf{\lambda})$,

\begin{widetext}
\begin{eqnarray} \label{likelihood_calculation}
	p(d|\bm{\lambda})
	&\propto& \exp\left(-\frac{1}{2}
	\langle d - (\mathcal{A}_{0} h^{0} + \mathcal{A}_{1} h^{1}) |
	d - (\mathcal{A}_{0} h^{0} + \mathcal{A}_{1} h^{1} \rangle \right) \\
	&\propto& \exp\left(
	  \langle d | \mathcal{A}_{0} h^{0} \rangle
	 - \frac{|\mathcal{A}_{0}|^{2}}{2} \langle h^{0} | h^{0} \rangle\right)
	 \times \exp\left(\langle d | \mathcal{A}_{1} h^{1} \rangle
	 - \frac{|\mathcal{A}_{1}|^{2}}{2} \langle h^{1} | h^{1} \rangle
	 \right) \nonumber \\
	&\propto&\Lambda_{\mathrm{np}} \times \Lambda_{\mathrm{p}}, \nonumber
\end{eqnarray}
\end{widetext}
%
where for simplicity we use the approximations that $\langle h^{0} | h^{1} \rangle = 0$ and 
that $h^{0}$ is the dominant harmonic, i.e., that the SNR in the $h^{0}$
harmonic is larger than in $h^{1}$. The calculation proceeds analogously when $h^{1}$ is
dominant, and can be extended to the general case by replacing $h^{1}$ by its projection onto the space orthogonal 
to $h^{0}$.
 We can therefore \emph{predict} the distribution for the precessing SNR $\rho_{p}$ by
 combining $\Lambda_{\mathrm{np}}(\mathbf{\lambda})$ computed from a non-precessing
parameter estimation analysis with an estimate for the precessing likelihood,

\begin{eqnarray} \label{eq:rho_p_likelihood}
	\Lambda_{\mathrm{p}}(\bm{\lambda})
	&\propto& \exp\left(
	 + \langle d | \mathcal{A}_{1} h^{1} \rangle
	 - \frac{|\mathcal{A}_{1}|^{2}}{2} \langle h^{1} | h^{1} \rangle
	 \right)  \\
	& \propto & \exp \left( - \frac{1}{2} \left( \tilde{\rho}_{p}^{2}(\bm{\lambda})
	- 2\hat{\rho}_{p} \tilde{\rho}_{p}(\bm{\lambda}) \cos \delta \phi_{JL}
	+\hat{\rho}_{p}^{2} \right) \right), \, \nonumber
\end{eqnarray}
%
where $\delta \phi_{JL} = \hat{\phi}_{JL} - \tilde{\phi}_{JL}(\bm{\lambda})$ is the difference between
the simulated and predicted values of the precession phase, $\hat{\rho}_{p}$ is the simulated value
of $\rho_{p}$ and $\tilde{\rho}_{p}$ is the \emph{informed} prior for the precession SNR. The majority
of parameters required to calculate the \emph{informed} prior are already given in the non-precessing results.
The two exceptions are the amplitude of the precessing spin $\chi_{p}$ and the
initial precession phase $\phi_{JL}$.  As discussed in Section \ref{ssec:q_chi},
we can obtain a prior for $\chi_{p}$ \textit{conditioned} upon the other
parameters, specifically the mass ratio and aligned spin $\chi_{\mathrm{eff}}$,
and this can be used to generate the informed prior on $\rho_p$.
The initial precession phase is unconstrained by the non-precessing parameter recovery,
so it is taken to be uniformly distributed. The \emph{predicted} posterior for $\rho_{p}$ can
then be calculated by marginalizing over the other parameters,

\begin{equation}\label{eq:p_rho_p}
	p(\rho_{p} | d) = \int d \delta \phi_{JL} \, d \tilde{\rho}_{p}
	\, p(\tilde{\rho}_{p} ) \,
	\Lambda_{p} \, ,
\end{equation}
%
where  $\delta \phi_{JL} $ can be analytically marginalised over, as explained in detail in Ref.~\cite{mills2020measuring}. 
By calculating the
\emph{predicted} posterior distribution for $\rho_{p}$ based upon a set of non-precessing samples,
we may examine the effect of other measured parameters on the final $\rho_p$ distribution.
For example, if the aligned-spin run favours a
binary that is close to equal mass and an orientation consistent with a face-on
system, then our prior belief will be that the precessing SNR will be low ---
it is only with unequal masses and systems misaligned with the line of sight
that there are significant precession effects in the observed waveform. A prior belief of
$\rho_{p}$ peaking at low values will cause the predicted $\rho_{p}$ to peak at values lower
than the simulated one and consequently so too will the inferred posterior distribution for
$\rho_{p}$ inferred from a full 15d parameter estimation analysis.

\begin{comment}



\charlie{back to the original}
In order to test this hypothesis, we would like to
\textit{predict}  the
distribution of the precessing SNR $\rho_{p}$ based upon the simulated value
and some informed priors. The prediction we are referring to is an 
 analytic estimate of the posterior distribution, where we estimate the likelihood contribution 
 from precession and generate the informed priors
 from the posterior distributions of a parameter estimation run with a non-precessing model. 
 These two components, the likelihood and the informed priors can then be combined to produce an estimate 
 or prediction for the posterior that would be generated if we sampled from the true posterior.  This allows us to 
 investigate the effect of other measured paramaters and priors on the final $\rho_p$ distribution.
 
 For example, if the aligned-spin run favours a
binary which is close to equal mass and an orientation consistent with a face-on
system, then our prior belief will be that the precessing SNR will be low ---
it is only with unequal masses and systems misaligned with the line of sight
that there are significant precession effects in the observed waveform. 

We will now examine this conjecture in detail.  The gravitational waveform,
in the two-harmonic approximation, is given by
%
\begin{equation}
  h = \mathcal{A}_{0} h^{0} + \mathcal{A}_{1} h^{1} \, ,
\end{equation}
%
where $h^{0, 1}$ and $\mathcal{A}_{0,1}$ implicitly depend upon the parameters $\bm{\lambda}$
of the system.  The frequencies of the harmonics are offset by the precession frequency.
Additionally, as shown in Figure \ref{fig:phenomd_vs_dominant}, the aligned-spin
waveform model recovers the dominant harmonic of the precessing waveform.

The likelihood is given in equation (\ref{likelihood_calculation}) and, substituting
the two-harmonic waveform, we obtain
%
\begin{widetext}
\begin{eqnarray} \label{likelihood_calculation}
	p(d|\bm{\lambda})
	&\propto& \exp\left(-\frac{1}{2}
	\langle d - (\mathcal{A}_{0} h^{0} + \mathcal{A}_{1} h^{1}) |
	d - (\mathcal{A}_{0} h^{0} + \mathcal{A}_{1} h^{1} \rangle \right) \\
	&\propto& \exp\left(
	  \langle d | \mathcal{A}_{0} h^{0} \rangle
	 + \langle d | \mathcal{A}_{1} h^{1} \rangle
	 - \frac{|\mathcal{A}_{0}|^{2}}{2} \langle h^{0} | h^{0} \rangle
	 - \frac{|\mathcal{A}_{1}|^{2}}{2} \langle h^{1} | h^{1} \rangle
	 \right) \nonumber
\end{eqnarray}
\end{widetext}
%
Thus we see that the likelihood factorizes into terms which depend only upon the
leading harmonic $h_0$ and terms which depend only on second harmonic $h_1$.
For simplicity, in this section we work in the approximation where $\langle h^{0} | h^{1} \rangle = 0$,
although the calculation can be extended, in a straightforward way, to the general case by
replacing $h^{1}$ by its projection onto the space orthogonal to $h^{0}$.  Additionally, we
will assume that $h^{0}$ is the dominant harmonic, i.e. that the SNR in the $h^{0}$
harmonic is larger than in $h^{1}$.  The calculation proceeds analogously when $h^{1}$ is
dominant.

The posterior probability density is obtained by multiplying the likelihood by the prior
probability distribution $p(\bm{\lambda})$ (see equation (\ref{bayesequation})) and the posterior
for a single parameter is obtained by marginalizing over the other parameters (equation (\ref{posteriorforoneparameter})).  Thus, we can obtain the posterior distribution for $\rho_{p}$
as
%
\begin{equation}\label{eq:rho_p_post}
	p(\rho_{p} | d) \propto \int d\bm{\lambda} \, p(\bm{\lambda}) \, p(d|\bm{\lambda})
	\delta(\hat{\rho}_{p} - \tilde{\rho}_{p}(\bm{\lambda}))
\end{equation}
%
where $\hat{\rho}_p $ is the \emph{true} (here true corresponds to the simulated value) value for the precession \ac{snr}, 
$\tilde{\rho}_{p}(\bm{\lambda})$ is the
precession \ac{snr} calculated from the parameters $\bm{\lambda}$
using Eq.~(\ref{rho_p}).

To investigate whether the observed parameters are leading to a systematic
bias of the precession SNR, we would like to predict the distribution for $\rho_p$
using \textit{only} parameter estimation results for a spin-aligned waveform
augmented by the expected value of $\rho_p$ taken from the simulated waveform.
The majority of the parameters
describing the precessing waveform are already given in the aligned-spin results.
The two exceptions are the amplitude of the precessing spin $\chi_{p}$ and the
initial precession phase $\phi_{JL}$.  As discussed in Section \ref{ssec:q_chi},
we can obtain a prior for $\chi_{p}$ \textit{conditioned} upon the other
parameters, specifically the mass ratio and aligned spin $\chi_{\mathrm{eff}}$,
and this can be used to generate the informed prior on $\rho_p$.
The initial precession phase is unconstrained by the non-precessing parameter recovery,
so it is taken to be uniformly distributed.


The likelihood can be factorized into contributions from the two harmonics,
%
\begin{equation}
	p(d|\bm{\lambda}) = \Lambda_{\mathrm{np}}(\bm{\lambda}) \cdot \Lambda_{\mathrm{p}}(\bm{\lambda})
\end{equation}
%
As already
mentioned, a spin-aligned parameter estimation run matches well with the dominant harmonic so we
use that to evaluate the non-precessing likelihood.  The precessing likelihood can be obtained
from equation (\ref{eg:likelihood_calculation}) as
%
\begin{eqnarray} \label{likelihood_prec}
	\Lambda_{\mathrm{p}}(\bm{\lambda})
	&\propto& \exp\left(
	 + \langle d | \mathcal{A}_{1} h^{1} \rangle
	 - \frac{|\mathcal{A}_{1}|^{2}}{2} \langle h^{1} | h^{1} \rangle
	 \right)  \\
	& \propto & \exp \left( - \frac{1}{2} \left( \tilde{\rho}_{p}^{2}(\bm{\lambda})
	- 2\hat{\rho}_{p} \tilde{\rho}_{p}(\bm{\lambda}) \cos \delta \phi_{JL}
	+\hat{\rho}_{p}^{2} \right) \right), \, \nonumber
\end{eqnarray}
%
\steve{check that the phase really is just the difference of $\phi_{JL}$s.}
where $\delta \phi_{JL} = \hat{\phi}_{JL} - \tilde{\phi}_{JL}(\bm{\lambda})$ is the difference between
the simulated and predicted values of the precession phase.

Substituting into the marginalized likelihood, equation (\ref{eq:rho_p_post}), we obtain
%
\begin{equation}\label{eq:p_rho_p}
	p(\rho_{p} | d) = \int d \delta \phi_{JL} \, d \tilde{\rho}_{p}
	\, p(\tilde{\rho}_{p} ) \,
	\Lambda_{p}(\hat{\rho}_{p}, \tilde{\rho}_{p}, \delta \phi_{JL}) \, ,
\end{equation}
%
where  $\delta \phi_{JL} $ can be analytically marginalised over, as explained in detail in Ref.~\cite{mills2020measuring}.

To avoid confusion with the previous definition of the conditioned prior (see for example Fig.~\ref{fig:conditioned_prior}), we refer to $p(\tilde{\rho}_{p} | d)$ as the \textit{informed} prior and use
the same definition for the conditioned prior as used in previous literature (see for example~\cite{Abbott:2020niy}).  The expression in equation (\ref{eq:p_rho_p}) makes it clear that the expected
distribution for $\rho_{p}$ is simply the product of the precessing likelihood with the
informed prior.  Thus, we have shown in detail that our conjecture is correct: the prior
expectation on the observability of precession (based, for example, on a spin-aligned parameter
recovery) will impact the distribution for the precession SNR.

\end{comment}
\subsection{Precessing signal}

\label{ssec:predict_prec}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{images/predicted_rho_p_from_PhenomD}
	\caption{
	Violin plot comparing the observed $\rho_{p}$ distribution (colored) from a precessing analysis,
	and the predicted distribution (white) based on the aligned-spin results and simulated value of $\rho_p$
	for the set of varying mass ratio simulations presented in Sec.~\ref{ssec:q_chi}.  The predicted and
	observed distributions for precession \ac{snr} are in good agreement, even though the $\rho_p$ in the
	simulated signal (red lines) lies above the peak of either distribution.
	}
	\label{fig:predicted_vs_inferred_rho_p}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{images/predicted_rho_p_from_PhenomD_prior_likelihood}
	\caption{
	The predicted distribution for the precession \ac{snr} $\rho_{p}$ (dashed orange) calculated as the product
	of the precessing contribution to the likelihood (black dotted line) and the informed prior of $\rho_{p}$ (blue) for the $q=4$ simulation presented in Sec.~\ref{ssec:q_chi}. For comparison, we show the inferred $\rho_{p}$ posterior distribution from the full 15 dimensional parameter estimation analysis (solid orange) and $\rho_{p}$ for the injection (red line).
	The informed prior is peaked at low values of $\rho_{p}$ causing the peak of the
	posterior to be smaller than the maximum likelihood value.
	}
	\label{fig:predicted_prior_rho_p}
\end{figure}

We now apply this conjecture to a precessing signal by attempting to \emph{predict} the posterior distributions for $\rho_p$.
This allows us to investigate how much our 
recovered posterior distributions may differ from the idealised case of a precession likelihood function distributed about the simulated (true) value.
We show the results of this for the mass ratio simulations presented in Sec.~\ref{ssec:q_chi} in Fig.~\ref{fig:predicted_vs_inferred_rho_p}. In Fig.~\ref{fig:predicted_prior_rho_p} we specifically focus on the $q=4$ simulation as this case has the largest $\rho_{p}$ and corresponds to a simulation where a non-precessing analysis is less justified. It is therefore a good case to show how the combination of the informed prior and the additional likelihood from precession $\Lambda_{\mathrm{p}}$ correctly estimates the large $\rho_{p}$.

In Fig.~\ref{fig:predicted_prior_rho_p} we show this predicted distribution, the informed prior, the $\chi^2$ likelihood function and the posterior distribution obtained from a full parameter estimation analysis.  By explicitly calculating the informed prior and likelihood terms separately for $\rho_p$,
we can see the effect of the prior on the $\rho_p$ posterior.
The prior strongly disfavours large
observable precession and therefore pulls the posterior towards \emph{smaller} values than the simulated value i.e. where the likelihood function peaks.

In Fig.~\ref{fig:predicted_vs_inferred_rho_p}, we show a comparison between the predicted and measured $\rho_{p}$ distributions for the set of runs with varying mass ratio presented in Sec.~\ref{ssec:q_chi}.  When we calculate the posterior, explicitly accounting for the parameter space weighting encoded in the informed prior on $\rho_{p}$, we find good agreement between the predicted and the inferred $\rho_{p}$ distributions and note that neither predicted nor inferred are centred around the \emph{true} value for the set of signals that we have simulated.  Of course, if we were to draw signals uniformly from the prior distribution, we would expect to observe the inferred distributions of $\rho_{p}$ matching with the simulated values.


==> results_psi.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.4]{vary_psi_chi_p_and_chi_p_prior}
	\includegraphics[scale=0.4]{vary_psi_violin_plot_network_precessing_snr}
	  \caption{Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior (left) and $\rho_p$ (right). Distributions are plotted for varying  $\psi_J$. Parameters other than $\psi_J$ match the ``standard injection'' (see Table~\ref{tab:standard_run})}
	\label{fig:chi_p_vs_psi}
\end{figure*}

The effect of changing the relative sensitivity to the two GW polarizations is clear from Eq.~(\ref{eq:zeta}).  Recalling that $\bar{b} = 0.11$ and $\theta_{JN} = 60^{\circ}$, we can express $\zeta$ (the ratio of the amplitudes of the two harmonics) as
%
\begin{equation}\label{eq:zeta_pol}
	|\zeta| = 0.15  \left|\frac{
	F_{+} + 2 i F_{\times} }{1 F_{+} + 0.8 i F_{\times} }\right|  \, , \nonumber
\end{equation}
%
Thus, $\zeta$, and consequently the imprint of precession on the waveform, will be maximized when the detector network is primarily sensitive to the $\times$ polarization and minimized when the network is sensitive to the $+$ polarization.  We can investigate this by varying the polarization angle of the simulated signal, in steps of $10\degree$ from the ``standard'' value of $40\degree$.  At $\psi = 40\degree$, the sensitivity to the two polarizations is approximately equal, $|F_{\times} |/|F_{+}| = 0.9$.  It is largest for $\psi = 20\degree$ where $|F_{\times}|/|F_{+}| = 25$ and smallest for $\psi=60\degree$ where $|F_{\times}|/|F_{+}| = 0.04$.  This leads to a variation in the precession \ac{snr} from $\rho_{p} \approx 3$ to $\rho_{p} \approx 7$.

In Fig.~\ref{fig:chi_p_vs_psi} we show the recovered posteriors for $\chi_p$ and $\rho_p$ for a set of runs where the precession is varied.
The precession \ac{snr} varies in accordance with expectation --- it is largest at $\psi = 20\degree$, where the median of the posterior is at $\rho_p = 6$ and there is no support for non-precessing systems, and smallest at $60\degree$ where the posterior extends down to $\rho_p = 0$.
The amount of observable precesssion directly impacts the inferred distribution for $\rho_p$.  For the $\psi = 60\degree$ signal, the posterior for $\chi_p$ is consistent with zero, or small in-plane spins, and large values are excluded.  Meanwhile for $\psi = 20\degree$, $\chi_p < 0.1$ is excluded while extremal in-plane spins are consistent with the observation.

\steve{can probably improve/strengthen this.}
It is well known that precession leaves a stronger imprint upon the $\times$ polarization.  However, we are not aware of previous results showing how simply changing the polarization of the system can so dramatically change the observable consequences of precession --- from being barely observable when the observed signal is primarily the $+$ polarization to being strongly observed in $\times$.  Using the two-harmonic approximation, we are able to straightforwardly predict this effect and then verify it with detailed parameter estimation studies.


==> results_sky.tex <==
\begin{table}[t]
    \begin{ruledtabular}
        \begin{tabular}{ c | c c c c c | c | }
            Label & $\mathrm{RA} / \mathrm{rad}$ & $\mathrm{DEC} / \mathrm{rad}$ & $\psi/{}^{\circ}$ & $d_{L}/\mathrm{MPc}$ & $\rho_{p}$ & $d_{L}/\mathrm{MPc}$ \\
            \hline
            A & 0.31 & 0.92 & 320 & 370 & 5.02 & $480^{+130}_{-180}$ \\
            B & 0.80 & 1.15 & 345 & 320 & 5.09 & $470^{+140}_{-160}$ \\
            C & 1.31 & 1.22 & 10 & 280 & 5.11 & $450^{+150}_{-160}$ \\
            D & 1.88 & 1.19 & 40 & 220 & 5.05 & $430^{+160}_{-160}$ \\
            E & 6.11 & 0.21 & 40 & 310 & 5.09 & $440^{+150}_{-170}$ \\
            \end{tabular}
        \end{ruledtabular}
    \caption{Table showing the simulated parameters for the sky location set (see Sec.~\ref{ssec:sky_loc}). All other parameters match the ``standard injection'' (see Table~\ref{tab:standard_run}). The recovered luminosity distance (far right column) is also shown.}
    \label{tab:sky_loc_runs}
\end{table}

We performed a series of runs where we altered
the sky location of the signal, keeping the masses
and spins of the components fixed.  We also maintained
the binary orientation $\theta_{\rm JN} = 60\degree$, but
varied the distance and polarization of the source to
ensure that the \ac{snr} remained constant and that the
relative contribution of the $+$ and $\times$ polarizations
was consistent with the standard run.
Furthermore, sky locations were restricted to those for which the relative
time of arrival between the Hanford and Livingston detectors
remains the same (i.e., we were sampling from the nearly
degenerate ring on the sky of constant time delays).
Details of the runs are given in Tab.~\ref{tab:sky_loc_runs}.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.7\textwidth]{skymap_comparison_for_varying_skyloc}
	\caption{
	Skymap showing the different simulated sky positions, see Table~\ref{tab:sky_loc_runs}. The solid lines
	show the 90\% credible intervals and the markers show the simulated sky position. Their respective colors
	matches their corresponding credible intervals. We vary the distance
	and polarization of the source to ensure that the \ac{snr} remains consistent with the standard
	injection in Table~\ref{tab:standard_run}.
}
	\label{fig:sky_loc}
\end{figure*}

Table~\ref{tab:sky_loc_runs} shows that the inferred luminosity distance
remains approximately constant despite the simulated luminosity distance varying by
almost a factor of two.  In addition, the recovered $\rho_p$ distribution remains
consistent with the ``standard'' injection.
Fig.~\ref{fig:sky_loc} shows that the inferred sky position of the source remains
essentially unchanged, and consistent with locations of the detectors' greatest sensitivity.
We note here that for this study we only considered the two detector LIGO network. 
Including VIRGO would likely have considerably improved the precision of the 
inferred sky location. We do not expect that this would affect any of the inferred
physical parameters or any of the main conclusions in this work.


==> results_snr.tex <==
We start with the fiducial run configuration described above and vary the
\ac{snr} of the simulated signal.

In the strong-signal limit, where the likelihood surface can be well approximated by 
a multivariate gaussian, it is well known that the accuracy with which parameters 
can be measured is generally
inversely proportional to the SNR~\citep{Cutler:1994ys, Poisson:1995ef}.  However,
this is not always the case due to, for example, degeneracies between parameters (see
Ref.~\cite{Vallisneri:2007ev} for a discussion of the limits of this approximation).

\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.4]{snr_chi_p}
	\includegraphics[scale=0.4]{snr_rho_p}
	\caption{ Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior (left) and $\rho_p$ compared to a non-central $\chi$ distribution with 2 degrees of freedom and non-centrality equal to the median of the $\rho_p$ distribution (right). Distributions are plotted for varying SNR. Parameters other than the \ac{snr} of the signal match the ``standard injection'' (see Table~\ref{tab:standard_run}).}
	\label{chi_p_vs_SNR}
\end{figure*}

Fig.~\ref{chi_p_vs_SNR} shows that as the \ac{snr} of the simulated signal increases, the accuracy and
precision of the inferred $\chi_{p}$ posterior distribution improves. As expected the width of the 90\%
credible interval decreases approximately linearly with increasing SNR. The improvement in the $\chi_{p}$
posterior distribution can be mapped to a linear increase in $\rho_{p}$.

When the simulated signal has low \ac{snr} ($\rho = 10$), the recovered $\chi_{p}$ posterior distribution
resembles the prior, implying that there is no information about precession in the data. For this case,
$\rho_{p}$ matches the expected distribution in the absence of any measurable precession --- a $\chi$
distribution with 2 degrees of freedom. As the \ac{snr} increases ($\rho = 20$-$30$), the 5th percentile of the
the $\rho_{p}$ distribution is comparable or greater than the $\rho_{p} = 2.1$ threshold. This maps
to the $\chi_{p}$ posterior distribution removing all support for near-zero $\chi_{p}$ ($\chi_{p}\lesssim 0.1$).
For larger SNRs ($\rho > 40$), the entire $\rho_{p}$ distribution is greater than the 2.1 threshold. This implies
significant power from precession. For these cases, we remove support for maximal precession
$\chi_{p} \sim 1$.

As expected we find good agreement between $\rho_{p}$ and a non-central $\chi$ distribution with 2 degrees
of freedom and non-centrality equal to the inferred power in the second harmonic (median of the $\rho_{p}$
distribution).


==> results_standard.tex <==
\begin{table*}[t]
    \begin{ruledtabular}
        \begin{tabular}{ l | c | c c | c c |}
            & Simulated &  \multicolumn{2}{c |}{Median} & \multicolumn{2}{c |}{maxL} \\
            \hline
           & Precessing & Non-Precessing & Precessing & Non-Precessing & Precessing \\
            Total mass $M / M_{\odot}$ & $40.0$ & $40^{+3}_{-2}$ & $40^{+4}_{-2}$ & $40.161$ & $40.507$ \\
            Chirp mass $\mathcal{M} / M_{\odot}$ & 16.22 & $16.5^{+0.3}_{-0.2}$ & $16.3^{+0.3}_{-0.3}$ & $16.459$ & $16.113$ \\
            Mass ratio $q$ & $2.0$ & $1.8^{+0.8}_{-0.7}$ & $1.9^{+0.9}_{-0.7}$ & $1.895$ & $2.191$ \\
            Inclination angle $\theta_{JN} / {}^{\circ} $ & $60.0$ & $110^{+50}_{-100}$ & $120^{+40}_{-90}$ & $30.0$ & $40.0$ \\
            Precession phase $\phi_{JL} / {}^{\circ}$ & $45.0$ & -- & $200^{+100}_{-200}$ & -- & $80.0$  \\
            Effective aligned spin, $\chi_{\mathrm{eff}}$ & $0.0$ & $0.044^{+0.099}_{-0.084}$ & $-0.005^{+0.098}_{-0.092}$ & $0.06$ & $-0.011$ \\
            Effective precessing spin, $\chi_p$ & $0.4$ &  -- & $0.5^{+0.4}_{-0.3}$ & -- & 0.554 \\
            Right ascension $\mathrm{RA} / \mathrm{rad}$ & $1.88$ & $3^{+3}_{-3}$ & $3^{+3}_{-3}$ & $1.418$ & $1.325$ \\
            Declination $\mathrm{DEC} / \mathrm{rad}$ & $1.19$ & $0.2^{+1.0}_{-1.2}$ & $0.2^{+1.0}_{-1.2}$ & $1.229$ & $1.221$ \\
            Luminosity distance $d_{L}/\mathrm{Mpc}$ & $223$ & $500^{+200}_{-200}$ & $400^{+200}_{-200}$ & $451.834$ & $372.706$ \\
            Network \ac{snr} $\rho$ & $20.0$ & $19.3^{+0.1}_{-0.2}$ & $19.7^{+0.2}_{-0.2}$ & $19.52$ & $19.936$ \\
            Precessing \ac{snr} $\rho_{p}$ & 5.05 & -- & $4^{+2}_{-2}$ & -- & $4.649$ \\
            \end{tabular}
        \end{ruledtabular}
    \caption{Table showing the simulated and inferred parameters for the ``standard'' injection when
    recovered by a non-precessing (\texttt{IMRPhenomD}) and a precessing (\texttt{IMRPhenomPv2}) waveform model.
    We report the median values along with the 90\% symmetric credible intervals and the maximum
    likelihood (maxL) value.
    }
    \label{tab:standard_run}
\end{table*}




We performed parameter estimation on the signal using the \texttt{LALInference}~\cite{Veitch:2014wba}
and \texttt{LALSimulation} libraries within \texttt{LALSuite}~\citep{LALSuite}. Parameter recovery was performed with the \texttt{IMRPhenomPv2} model~\citep{Bohe:PhenomPv2, Hannam:2013oca},
which matches the simulated signal to remove any systematic error caused by waveform uncertainty,
and the corresponding \texttt{IMRPhenomD} aligned-spin waveform model~\citep{Khan:2015jqa, Husa:2015iqa},
which does not include any precession effects. Additionally, all analyses used exactly the same priors as those used in the LIGO-Virgo discovery papers, for details, see Appendix B.1 of~\citep{LIGOScientific:2018mvr}. All post-processing was handled by the \texttt{PESummary} python
package\citep{Hoy:2020vys}.

Tab.~\ref{tab:standard_run} summarises the key results for the standard configuration.
All uncertainties are the 90\% symmetric credible intervals.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{images/phenomD_vs_dominant}
	\caption{Comparison of the simulated precessing (green), non-precessing maximum likelihood (red), precessing maximum likelihood (black) and dominant precessing harmonic (blue) waveforms as a function of frequency. Waveforms are projected onto the LIGO Hanford detector.
  }
	\label{fig:phenomd_vs_dominant}
\end{figure}

We begin by comparing the overall differences between parameter recovery with the precessing, \texttt{IMRPhenomPv2}, and non-precessing, \texttt{IMRPhenomD}, runs.  From the table, we see that the maximum likelihood \ac{snr} for the non-precessing model is, as expected, lower than for the precessing waveforms.  This can be easily understood from the two-harmonic approximation.  Since the precessing waveform is well approximated by the sum of two non-precessing harmonics, we would expect the non-precessing recovery to accurately recover the more significant of these two.  If that were the case, the we would expect that,
%
\begin{equation}
	\rho_{D}^{2} \approx \rho^{2} - \rho_{p}^{2},
\end{equation}
%
and this is indeed the case, as $\rho_{D} = 19.52$, $\rho = 19.94$
and the recovered power in the second harmonic is $\rho_p = 4.6$.
Furthermore, we see that the recovered waveforms confirm this expectation: the recovered waveform when we
include precession matches well with the simulated signal, while the non-precessing run recovers a waveform that
 matches the dominant harmonic, as show in Fig.~\ref{fig:phenomd_vs_dominant}.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{images/phenom_D_P_compare_2d_contour_plot_mass_ratio_and_chi_eff}
	\includegraphics[width=0.49\textwidth]{images/phenom_P_D_2d_contour_plot_theta_jn_and_luminosity_distance}
	\caption{2d contour comparing $q$--$\chi_{\mathrm{eff}}$ (left) and distance--inclination (right) degeneracies when precession effects are included.
  Contours show the 90\% confidence interval. Bounded two-dimensional \acp{kde} are used for estimating the joint probability density.  The black circle indicates the simulated values.}
	\label{fig:p_vs_d_degeneracy_contour}
\end{figure*}

We first consider the accuracy with which the masses and (aligned) spins are recovered.  As expected, the chirp mass
of the system is well recovered, in that it matches the simulated value with only a 2\% uncertainty, which remains constant for both precessing and non-precessing runs.  As is well known, there is a degeneracy between mass-ratio and spin,
particularly during the inspiral part of the waveform \cite{Poisson:1995ef, Baird:2012cu, farr2016parameter, ng2018gravitational}, which leads to significant uncertainty in both
parameters.  In Fig.~\ref{fig:p_vs_d_degeneracy_contour} we show the recovery of the mass ratio and spin, for both precessing and non-precessing runs.  When the model used to recover includes precession effects, the peak of the posteriors is located close to the simulated value ($\chi_\mathrm{eff} = 0$ and $q = 2.0$) and, while the degeneracy leads to significant uncertainty in both parameters, the mass-ratio distribution is clearly peaked away from $q=1$.  Interestingly, when we recover with a non-precessing waveform model, the inferred \textit{aligned} spin component is systematically offset, with a peak at $\chi_{\mathrm{eff}} \approx 0.05$.  This can be understood by recalling that precession induces a secular drift in the phase evolution of the binary, and this can be mimicked by a change in the value of the aligned spin \cite{Apostolatos:1994mx, Fairhurst:2019_2harm}.
This discrepancy has not been seen in LIGO/Virgo observations~\citep{LIGOScientific:2018mvr} as we have
not observed any systems with significant $\rho_{p}$ (see Fig.~\ref{currentdetections}). We investigate this
further in Sec.~\ref{ssec:q_chi}, where we study the effect of varying the mass ratio.

For non-precessing binaries, it is generally not possible to accurately recover the distance and orientation of the source, due to a well known degeneracy (see e.g., Ref.~\cite{Usman:2018imj} for details), although the observation of higher signal harmonics can break this degeneracy through an independent measurement of the source inclination~\citep{Cutler:1994ys, Usman:2018imj, kalaghatgi2019parameter}.  Similarly, the observation of precession can break this degeneracy~\citep{vitale2018measuring}. Precession causes an oscillation of the orbital plane leading to a time-dependence of the orientation of the orbital plane relative to the line of sight.  Equivalently, in the two-harmonic picture, precession leads to the observation of a second harmonic and, consequently, additional constraints on the binary orientation as the amplitudes of the harmonics depend upon the viewing angle. In
Fig.~\ref{fig:p_vs_d_degeneracy_contour}, we show the inferred two-dimensional distance and inclination posteriors for the precessing and non-precessing runs.
As expected, the precessing run constrains the source to be away from face-on,
while the non-precessing run simply returns the prior.  However, even with observable precession, the simulated distance and orientation are not accurately recovered --- a significant fraction of the posterior support is for a system at a greater distance and oriented closer to face-on. We will see how these measurements improve with stronger precession
in Sec.~\ref{ssec:chi_p}.

The sky location of the source is not well recovered.  The analysis was performed with only the two LIGO detectors, and therefore we expect to recover the source restricted to a ring on the sky, which corresponds to a fixed time delay between the detectors \cite{Fairhurst:2009tc, Singer:2015ema}.  The location along the ring cannot be well constrained and, as expected the inferred location is preferentially associated with sky positions where the detector network is more sensitive.  Thus, while the simulated sky location is within the 90\% region, it is not at or close to the peak.  This impacts the recovery of the distance, with the signal being recovered at larger distances, although the simulated distance remains within the 90\% range.  In Section \ref{ssec:sky_loc}, we show results from a set of runs with varying sky location, and verify that at sky locations where the network is more sensitive, the distance posterior is more consistent with the simulated value.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{corner_chip_rhop_thetajn_phijl}
	\caption{A corner plot showing the recovered values of binary orientation $\theta_{JN}$, precessing spin $\chi_{p}$, precession phase $\phi_{JL}$ and precession \ac{snr} $\rho_{p}$.  Shading shows the $1\sigma$, $3\sigma$ and $5\sigma$ confidence intervals. Black dots show the simulated values. The grey histograms show the \emph{informed} prior, see Sec.~\ref{sec:rho_p_predict}. There is a clear correlation between the binary orientation and inferred precession spin, with signals which are close to face on ($\cos \theta \approx \pm 1$) having larger values of precessing spin, while those which are more inclined having less precessing spin.  The precession \ac{snr} only weakly correlated with $\chi_p$.}
	\label{fig:rho_p_chi_p}
\end{figure}

Lastly, we turn to measurement of precession.  In Fig.~\ref{fig:rho_p_chi_p} we show the recovered distributions for
binary orientation, $\theta_{JN}$, precessing spin $\chi_{p}$, initial precession phase, $\phi_{JL}$, and precession
SNR, $\rho_{p}$.
There is a clear correlation between the inferred orientation and $\chi_p$, with binaries that are more
inclined having lower values of $\chi_p$.  Neither of these quantities are directly observable, it
is only the amount of observable precession in the system, encoded by $\rho_p$, that can be measured.  Thus the orientation
and spin must combine to give the right amount of power in precession, and we see that this is the
case --- there is little correlation between the recovered values of $\rho_p$ and the precessing spin $\chi_p$.
The inferred value of the precessing spin $\chi_{p}$ and precession \ac{snr} $\rho_p$ are both consistent with the
simulated values.  Specifically, the signal has $\chi_p = 0.4$ and this is consistent with the recovered value, although the
posterior distribution is broad, with support over essentially the entire range from 0 to 1. The precession \ac{snr} peaks
well away from zero, giving clear indication of precession in the system. However, the peak of the distribution
occurs at 3.5, while the simulated value is 5.0.  We have deliberately chosen an event with
significant observable precession. Only a small fraction of the parameter-space volume leads to such significant
precession as shown by the \emph{informed} prior on Fig.~\ref{fig:rho_p_chi_p}. This is calculated by estimating the allowed values of $\rho_{p}$ conditioned on the measurements from a non-precessing
analysis. See Sec.~\ref{sec:rho_p_predict} for further details.

The precession phase, $\phi_{JL}$, while not measured with great accuracy, does show two peaks, which are
consistent with the simulated value of $45\degree$ ($0.8$ rad).  The precession phase can be inferred from the
relative phase of the two precessing harmonics using Eq.~(\ref{eq:zeta}), provided the binary
orientation is well measured.  There is a clear dependence with the binary orientation:
if $\theta_{JN} < 90\degree$ then the peak is in $\phi_{JL}$ at the simulated value and if it is greater then $\phi_{JL}$ is offset by
$180\degree$, to compensate for the change in sign of the $\cos \theta_{JN}$ terms in Eq.~(\ref{eq:zeta}).


==> results_total_mass.tex <==

\begin{figure*}[t]
  \centering
	\includegraphics[scale=0.4]{M_and_chi_p_prior.pdf}
	\includegraphics[scale=0.4]{total_mass_rho_p.pdf}
    \caption{Violin plots showing the recovered posterior distributions distributions for $\chi_p$ compared to its prior (left) and $\rho_p$ (right). Distributions are plotted for varying total mass. Parameters other than the total mass of the signal match the ``standard injection'' (see Table~\ref{tab:standard_run})}
  \label{chi_p_vs_m}
\end{figure*}


We now vary the total mass of the system, keeping all other parameters including mass ratio fixed, in steps of
$20\,M_\odot$.  As before, we keep the \ac{snr} of the system constant at 20, so the higher mass systems are
generated at a greater distance.  The inferred distributions for $\chi_p$ and $\rho_p$ are shown in Fig.~\ref{chi_p_vs_m}.

As the total mass of the source increases, the length of the waveform decreases, as does the
number of precession cycles, with the number scaling approximately inversely to the total mass (see Eq.~(45) of \citep{Apostolatos:1994mx}).
From the two-harmonic perspective, a small number of precession cycles leads to a large overlap between the harmonics.
Specifically, for the $M=100 M_{\odot}$ system
the overlap between the normalised harmonics is $\langle \hat{h}_0| \hat{h}_1 \rangle = 0.77$, where $\hat{h} = h/|h|$
and the inner product is defined in Eq.~(\ref{eq:inner_prod}).  At $M=20M_{\odot}$, the harmonics are close to orthogonal
with $\langle\hat{h}_0| \hat{h}_1 \rangle = 0.15$.  The opening angle doesn't change significantly, with $\bar{b} = 0.14$ at $M=20 M_{\odot}$
and $\bar{b} = 0.21$ at $M=100 M_{\odot}$.

At lower masses, $ M \le 40 M_{\odot}$, while the precessing spin is not tightly
constrained, it is clearly restricted to be non-zero and the precession \ac{snr} has
essentially no support for $\rho_p = 0$.  For the $60 M_{\odot}$ and $80 M_{\odot}$
mergers, the precessing spin is still peaked close to the simulated value while
$\rho_p$ peaks above 2.1 showing evidence for observable precession, although both $\rho_p$ and
$\chi_p$ distributions do extend to zero.

For the high-mass system,
$M = 100 M_{\odot}$, the $\chi_p$ posterior more closely matches the prior and we are unable
to exclude $\chi_p = 0$. The inferred $\rho_{p}$ distribution peaks close to
zero, and is consistent with no precession, even though the precession \ac{snr} in
the simulated signal is
similar to the lower mass signals.  This is likely due to the breakdown of the
two-harmonic approximation for this short signal.  In particular, for a high-mass system, the power
orthogonal to the leading harmonic will depend sensitively upon the initial
precession phase $\phi_{JL}$.  The fact that the recovered value of $\rho_p$ is
inconsistent with the simulated value may be due to this fact: the value of $\phi_{JL} = 45^{\circ}$
used in the simulation leads to maximal observable precession.  Across the
full parameter space there are very few configurations with significant precession, so
this observation is dis-favoured by our priors.  We explore the prior effects such as this in detail in Sec.~\ref{ssec:predict_np}.


==> results_verification.tex <==

\begin{figure}[t]
        \centering
        \includegraphics[scale=0.4]{rho_p_in_absence_of_precession}
        \caption{Distribution of $\rho_{p}$ in the absence of precession for the ``standard injection''.  The inferred $\rho_{p}$ distribution using the {\sc{IMRPhenomPv2}} approximant for recovery is shown by the solid orange line. The dashed orange line shows the predicted distribution using samples collected from an aligned-spin analysis and setting the simulated precession \ac{snr} to be 0.}
        \label{fig:rho_p_in_absence_of_precession}
\end{figure}

We now look at the expected posterior distribution for $\rho_p$ when there is no precession in the the signal.  In  
Ref.~\cite{Fairhurst:2019_2harm} it was shown that under gaussian noise and in the absence of any precession, the distribution for $\rho_p$  is a $\chi^{2}$ distribution with two degrees of freedom. This then led to the natural heuristic that $\rho_p = 2.1$ should be the threshold for observable precession. Deriving this distribution in this way is equivalent to calculating the likelihood in Eq.~(\ref{eq:rho_p_likelihood}) with zero precession ($\hat{\rho}_{p} = 0$). Using Eq.~(\ref{eq:p_rho_p}) we can now improve upon this and obtain a more accurate estimate of the expected posterior distribution in the absence of precession. We do this by using parameter estimation samples from an aligned-spin model and setting the simulated precession \ac{snr} to be 0, this then allows us to account for the effects of priors and different noise realisations.

In Fig.~\ref{fig:rho_p_in_absence_of_precession} we show the predicted and observed distributions for the precession \ac{snr} for a non-precessing signal.
We use a non-precessing equivalent of the ``standard'' injection as our simulated signal (i.e., we set
$\chi_{p}=0$ while ensuring all other parameters match those in Tab.~\ref{tab:standard_run}). We inject with zero noise and use the
{\texttt{IMRPhenomPv2}} model for parameter recovery.

The inferred $\rho_{p}$ distribution is peaked at lower values that the prediction from the likelihood (the $\chi^2$ distribution with 2 degrees of freedom).  However, the informed prior on $\rho_p$, which is shown in Fig.~\ref{fig:predicted_prior_rho_p}, is peaked at $\rho_p \lesssim 1$, and this leads to the predicted posterior on $\rho_p$ also favouring lower values.  When we combine the likelihood, based on the simulated value of $\rho_p$, with the informed prior we are able to accurately predict the $\rho_p$ posterior \textit{without} performing parameter estimation incorporating precession.

The distribution for the informed prior on precession \ac{snr} will depend upon the details of the signal.  In particular, it will be strongly peaked near zero for events that are likely to have small opening angle (eqivalently $\bar{b}$), i.e.,~events that are close to equal mass and have significant spin aligned with the orbital angular momentum, while high mass-ratio events and those with large anti-aligned spins will lead to greater support for large values of $\rho_p$.  Furthermore, for binaries where the orientation can be well measured, \textit{without} precession information, for example where higher modes are important, those that are close to face-on will lead to predictions of smaller $\rho_p$ while those that are edge-on will give larger values.  Given that the majority of signals observed to date are consistent with equal mass binaries, in most cases the prior on $\rho_p$ will tend to be peaked at low values.  Consequently, the simple threshold of $\rho_p \gtrsim 2.1$ as evidence for precession, remains appropriate and is likely more stringent than suggested by the simple likelihood calculation.


==> setup.tex <==
We begin by describing the results of the parameter recovery routine for a specific simulated signal.  The details of the signal are given in Tab.~\ref{tab:standard_run}.  These parameters were chosen so that precession effects would be significant in the observed waveform while still being consistent with the observed population of \ac{bbh}s.  In the following sections, we vary over the parameters of the signal one-by-one to investigate the impact of each parameter on the observability of precession and the accuracy of parameter recovery.  For each parameter, we are able to both increase and decrease the significance of precession.

% The parameters of our standard configuration are chosen as follows.
By taking the inferred properties of the \ac{bbh}s observed in the first, second and third
observing runs~\citep{Abbott:2020niy}, it is predicted that 90\% of detected binaries will have mass ratios
$q < 4$ and $\sim 97\%$ of \acp{bh} in these binaries will have masses less than
$45M_{\odot}$~\citep{Abbott:2020gyp}. 
Our ``standard'' simulated signal was chosen to have total mass $M = 40 M_{\odot}$ and
mass ratio $q = 2$ inclined at an angle of $\theta_{JN} = 60^{\degree}$. This corresponds to component masses of $26.7 M_{\odot}$ and $13.3 M_{\odot}$. This mass ratio and inclination 
was chosen to increase the observability of precession.
%, so in that sense these results are in general
%more favourable to precession measurement than typical observations.

Of the 50 events reported by the LIGO/Virgo, 13 exclude the aligned-spin measure $\chi_{\mathrm{eff}} = 0$ at 90\% confidence~\cite{LIGOScientificCollaborationandVirgoCollaborationGW151226ObservationGravitational2016, LIGOScientific:2018mvr, Abbott:2020niy}. The other 37 observations peak at
$\chi_{\mathrm{eff}} = 0$~\citep{LIGOScientific:2018mvr, Abbott:2020niy}. Based on this, studies have shown that
it is likely \acp{bh} in binaries have low spin
magnitudes~\citep{LIGOScientific:2018jsj, Farr:2017uvj, Tiwari:2018qch, Fairhurst:2019srr}. For this reason,
in our standard configuration the \ac{bh} spins were chosen such that there is zero spin aligned with the binary's
orbital angular momentum, $\chi_{\mathrm{eff}} = 0$. We introduce precession by giving the more massive \ac{bh} a
spin of $0.4$ in-plane and leaving the second \ac{bh} with zero spin; two-spin effects are generally far weaker than the
dominant precession effect, which exhibits the same phenomenology as a single-spin 
system~\cite{Buonanno:2004yd,Schmidt:2014iyl}. From Eq.~(\ref{chi_p}) we see that this
gives us a system with $\chi_{p} = 0.4$.
The opening angle for the binary when the signal enters the detector's sensitivity
band is $10^{\circ}$ and the average value of the parameter $b = \tan(\beta/2)$ is $\overline{b}=0.11$, from Eq	.~(\ref{eq:b_bar}).  The
signal is simulated using the \texttt{IMRPhenomPv2} waveform model that incorporates precession effects,
but not higher harmonics ($\ell > 2$) in the signal~\cite{Hannam:2013oca, Bohe:PhenomPv2}.

Our ``standard'' simulated signal was chosen to be more favourable to precession measurements than typical LIGO-Virgo observations. Assuming systems are distributed uniformly in binary orientation, masses drawn from a power law distribution and spins drawn from a low isotropic distribution (see Ref.~\cite{Fairhurst:2019srr} for details), we expect that 4 in every 100 binaries detected by LIGO-Virgo will be inclined at angles greater than $60^{\degree}$ and have $\overline{b} > 0.11$.

The sky location of the binary was chosen to have $\text{RA} = 1.88 \,\text{rad}, \text{DEC}=1.19\, \text{rad}$.
The coalescence time is $t = 1186741861$ GPS (corresponding to the merger time of
GW170814~\citep{abbott2017gw170814}). The polarization angle, defined by the orientation of the orbital
plane when entering the sensitive band at $20\mathrm{Hz}$, is  $\psi = 40\degree$. The two harmonic
approximation is calculated in the J-aligned frame ($\hat{z} = \hat{\mathbf{J}}$). In this frame, the polarization
angle is $\psi_{J} = 120\degree$, which gives antenna factors for H1 of $F_{+}=0.34$ and $F_{\times}=0.53$
and for L1 of $F_{+}=-0.45$ and $F_{\times}=-0.30$, thus both detectors are roughly equally sensitive to
the two GW polarizations.

We injected the signals
into zero noise. The zero-noise analysis results will be similar to those obtained from the average results of
multiple identical injections in different Gaussian noise realisations. The simulated signal is recovered using
the LIGO Livingston and Hanford detectors with sensitivities matching those achieved in the second observing
run (O2) \cite{LIGOScientific:2018mvr}. A low frequency cut-off of
$20$Hz was used for likelihood evaluations, this frequency is also used as the reference frequency when defining 
all frequency dependent parameters such as $\theta_{JN}$.
  Both the LIGO Livingston and Hanford sensitivities improved
prior to the \ac{O3} ~\citep{buikema2020sensitivity} and are expected to improve further prior to the fourth observing
run (O4)~\citep{abbott2018prospects}. The results presented in this work are unlikely to be affected significantly 
by these changes and therefore we expect the main conclusions to be valid for O4 and beyond. 

The \ac{snr} of the signal is
fixed to be 20, corresponding to a moderately loud signal for aLIGO and AdV
observations~\citep{abbott2018prospects}. This sets the distance to $d_L = 223$\,Mpc.
The simulated \ac{snr} in the two
detectors is 16.2 in L1 and  11.7 in H1.  The simulated precession \ac{snr} in each of the detectors is 3.7 and 3.4
respectively, giving a network  precession \ac{snr} of 5.0.  Thus, we expect that precession will be clearly observable in
this signal.

